Covering Simple Orthogonal Polygons with Rectangles

We study the problem of Covering Orthogonal Polygons with Rectangles. For polynomial-time algorithms, the best-known approximation factor is $O(\sqrt{\log n})$ when the input polygon may have holes [Kumar and Ramesh, STOC '99, SICOMP '03], and there is a $2$-factor approximation algorithm known when the polygon is hole-free [Franzblau, SIDMA '89]. Arguably, an easier problem is the Boundary Cover problem where we are interested in covering only the boundary of the polygon in contrast to the original problem where we are interested in covering the interior of the polygon, hence it is also referred as the Interior Cover problem. For the Boundary Cover problem, a $4$-factor approximation algorithm is known to exist and it is APX-hard when the polygon has holes [Berman and DasGupta, Algorithmica '94]. In this work, we investigate how effective is local search algorithm for the above covering problems on simple polygons. We prove that a simple local search algorithm yields a PTAS for the Boundary Cover problem when the polygon is simple. Our proof relies on the existence of planar supports on appropriate hypergraphs defined on the Boundary Cover problem instance. On the other hand, we construct instances where support graphs for the Interior Cover problem have arbitrarily large bicliques, thus implying that the same local search technique cannot yield a PTAS for this problem. We also show large locality gap for its dual problem, namely the Maximum Antirectangle problem.

==> sections/proof-induction-v0.tex <==
\section{Existence of Planar Boundary Supports}

We shall denote the set of all area-maximal rectangles in a simple orthogonal polygon $P$ by $\RR^K(P)$. We will first prove two easy cases and then use them to prove the main theorem.

\begin{theorem}
  \label{thm:main}
  Given a simple orthogonal polygon $P$ and a set of area maximal rectangles $\RR$ with respect to $P$, there exists planar support graphs for $(\RR,\dP)$.
\end{theorem}

\begin{definition}[Star family]
  A family of rectangles $\RR$ and a polygon $P$ are said to be a star family if the following holds:
  \begin{enumerate}
  \item $\RR = \{R_1,\dots, R_t, R_c\}$ where if $R_i \cap R_j \neq \emptyset$ then $R_i \cap R_j \subseteq R_c$, for $1 \le i < j \le t$. We refer $R_c$ as the center rectangle of the star family.
  \item Every rectangle in $\RR$ is area-maximal with respect to $P$.
  \end{enumerate}
\end{definition}

See Figure so-and-so for an example of a star family.

\begin{lemma}
Every star family has a boundary support that is a star graph.
\end{lemma}

\begin{lemma}
  \label{lem:etoile-sans-centre}
Every star family without its center rectangle, i.e. $(\RR\setminus R_c, \dP))$, has a planar support.
\end{lemma}

\begin{lemma}
  \label{lem:hereditary-planar}
  Given a simple orthogonal polygon $P$ and a set of area-maximal rectangles $\RR$ with respect to $P$. If $(\RR,\dP)$ has a planar support then for every $\RR' \subset \RR$, $(\RR',\dP)$ also has a planar support.
\end{lemma}

\begin{proof}
  We borrow the ideas of the left-right planarity test, attributed to de Fraysseix, Rosenstiehl, and de Mendez \cite{}.
  A finite graph $G$ is planar iff there exists a $F$-coloring of the cotree edges with respect to a depth-first-tree $T$ on $G$.
  If for every $v \in V$ and outgoing edges $e_i$ and $e_j$ from $v$, the following two condition are satisfied.
  \begin{itemize}
  \item
    All return edges of $e_i$ ending strictly higher than $lowpt(e_j)$ belong to one class, and
  \item
    All return edges of $e_j$ ending strictly higher than $lowpt(e_i)$ belong to the other class.
  \end{itemize}

  We are given a planar support graph $G$ for $(\RR,\dP)$. We claim that for every $R \in \RR$, there exists a planar support graph $G'$ for $(\RR\setminus\{R\},\dP)$.

  Consider a DFS tree $T$ defined on $G$ rooted at $v_R$. As $G$ is planar there exists a left-right coloring of the cotree edges. For all the cotree edges $(x_{i,j},v)$ that points from $x_{i,j}$ and return to $v$, where $x_{i,j}$ is in a subtree rooted at $w_i$, where $w_i$ is a child of $v$ in $T$. We replace the edge $(x_{i,j}, v)$ by $(x_{i,j}, w_i)$ retaining the color class of this new cotree edge. We call this replacement operation \emph{shortcutting}.

  For every $p \in dP$, if $\RR_p$ lies in some subtree rooted at $w_i$, for some $i \in [t]$, then $\RR_p$ is supported by this shortcutting. If $\RR_p$ is distributed across subtrees rooted at multiple children of $v$ then we claim that we can connect the vertices $\{w_i | i \in [t]\}$ such that $\RR_p$ is supported. Note we can ignore the descendants of $w_i$, for every $i \in [t]$ and only consider the children of $v$ in order to support $\RR_p$.

  \begin{enumerate}
  \item $\cup_{i \in [t]}R(w_i) \subset P$. Let $P' := \cup_{i \in [t]}R(w_i)$. $P'$ has complexity strictly smaller than $P$. We inductively argue that  $(\cup_{i \in [t]}R(w_i), \dP')$ has a planar support.
    
  \item $\cup_{i \in [t]}R(w_i) = P$.
    This precisely an instance of star family without the center rectangle. In our case, the center rectangle is $R(v)$. From Lemma~\ref{lem:etoile-sans-centre}, $(\cup_{i \in [t]} R(w_i), \dP)$ has a planar support. For every distict $i, j \in [t]$ the vertices in the subtrees rooted at $w_i$ and $w_j$ are independent, hence the subtrees can be independently drawn.
    
  \end{enumerate}
  
  Let this new graph be called $G'$.

  It is obvious, that the cotree edges in $G'$ have an $F$-coloring, thus $G'$ is planar.

  What remains to be proven is that $G'$ is a support graph for $(\RR\setminus\{R\}, \dP)$. To that end, consider a point $p \in \dP$. We claim that $G[\RR_p\setminus\{R\}]$ is connected. If $R \notin \RR_p$ there is nothing to prove.
  We assume that $R \in \RR_p$ without loss of generality and $\RR_p$ contains at least one other rectangle other than $R$. Also, note that the vertices corresponding to $\RR_p$ lies only in a subtree rooted at one of the children of $v$. 
\end{proof}

\begin{definition}[Horizontal R-Tree \cite{}]
  Given a simple orthogonal polygon $P$, we horizontally cut $P$ along all its concave corners. This partitions $P$ into a set of interior disjoint rectangles $R_1,\uplus\dots,\uplus R_m$. We define a graph $T(P) = (V_T,E_T)$ where we have a vertex $v_i$ corresponding to $R_i$, for every $1\le i \le m$, and $(v_i,v_j) \in E_T$ if $\partial R_i \cap \partial R_j \neq \emptyset$.
\end{definition}

\begin{lemma}
Given a simple orthogonal polygon $P$, $T(P)$ is a tree.
\end{lemma}


\begin{definition}[Complexity of an Orthogonal Polygon]
  Given an orthogonal polygon $P$, the complexity of $P$ is the number of corners $P$ has including both convex and concave corners. We shall refer this qauntity by $|P|$.
\end{definition}

\begin{definition}[Pocket of a Simple Orthogonal Polygon]
  Given a simple orthogonal polygon $P$, we say a rectangle $R$ to be a pocket of $P$ if the following conditions hold. See Figure...
  \begin{enumerate}
    \item
      $R \subset P$,
    \item
     % $P\setminus\pock(P)$ is a simple polygon
      $|P| - |P\setminus R| \in \{2,4\}$, and %TODO: define |P| as the number of corners of $P$.
    \item
      exactly one side of $R$ is contained in $\partial(P\setminus R)$.
  \end{enumerate}

  The side of pocket $R$ that is contained in $\partial(P\setminus R)$ is called the top side $t$ of $R$. Accordingly, its opposite side is called the bottom side $b$ of $R$. On traversing $\partial R$ in clockwise direction, the side that appears after top and before bottom is the right side $r$ and its opposite side is the left side $\ell$.
%  is a \emph{good} sub-polygon of $P$, if $P'$ is connected and $P\setminus P'$ is a rectangle. %, and the projection of $P\setminus P'$ on the opposite side of $\dP$ is orthogonally monotonic. Also, the complexity of $|P'| = |P| - x$, where $x \in \{2,4 \}$.
\end{definition}

\begin{lemma}
  \label{lem:pocket}
  Every simple orthogonal polygon that is not a rectangle has a pocket.
\end{lemma}

%\begin{lemma}
%Given $P$ and a good sub-polygon $P' \subset P$, $\RR^K(P') \subset \RR^K(P)$.
%\end{lemma}
\begin{definition}[Extremal side of a Simple Orthogonal Polygon]
\end{definition}

Let $v$ be a leaf in $T(P)$. Then $\RR_v$ be the set of rectangles whose bottom blocker is the bottom side of $v$.
Invariants: 
\begin{enumerate}
  \item
    $G[\RR_v]$ is a tree.
  \item
    If $v$ is a leaf of $T(P)$ then $\RR_v$ appears on the outer face of the plane graph $G$.
\end{enumerate}

  

\begin{lemma}
  Given a simple orthogonal polygon $P$ and let $\RR^K(P)$ be the set of all area-maximal rectangles with respect to $P$.
   $(\RR^K(P),\dP)$ has a planar support. Furthermore, there is a plane graph of the support such that the vertices corresponding to the vertically-blocked rectangles of $P$ are in its outer face.
\end{lemma}

\begin{proof}
  %We identify a pocket $\pock(P)$ and let $P':= P\setminus\pock(P)$
  %Given a planar drawing of the support of $(\RR^K(P'),\dP')$. We maintain an invariant that for every extremal side of $\dP'$ there exists a drawing such that all rectangles that intersect that extremal side are present in the outer face of the drawing.

  %We prove the statement of Lemma... inductively on the complexity of $P$. The base case is when $|P| = 4$, i.e., $P$ is a rectangle and $\RR^K(P)$ is $\{P\}$. Hence, the support graph comprises of a single vertex.

  %Let $|P| > 4$. From Lemma~\ref{lem:pocket}, we know $P$ has a pocket $A$. Let $P' := P \setminus A$.

  We consider $T(P)$, the horizontal R-Tree of $P$. We prove inductively on the number of vertices of $T(P)$.
  The base case is when there is a single vertex in $T(P)$, i.e., $P$ is a rectangle and the claim of the lemma is trivially true.
  
  Let $A \subset P$ be rectangle that corresponds to a leaf of $T(P)$.
  Let $P' := P \setminus A$. Also let $B$ be the parent of $A$.
  The inductive hypothesis is if the statement of the lemma is true for $P'$ then it is also true for $P$.

  The high-level idea is to attach the vertices of $\RR_A$ to some of the vertices of $\RR_{B}$ and also remove some of the subtrees at $\RR_B$ and attach it to vertices in $\RR_A$.

  As every rectangle $R \in\RR_A$ has the bottom side of $A$ as its bottom blocker, therefore from Lemma~\ref{lem:opp-blockers}, $R$ can be uniquely determined by its top blocker. Similarly, every rectangle in $\RR_B$ can be uniquely determined by its top blocker.

  Thus, for every $R \in \RR_A$, if $R_x \subseteq B_x$ then there exists a unique $R' \in \RR_B$ such that $R$ and $R'$ have a common top blocker. We say $R'$ is an image of $R$.

  There are two cases: given $R \in \RR_A$ either $R'\in \RR^K(P)$ or not.
  We say $R \in \RR_A$ is a Type-1 rectangle if $R' \in \RR^K(P)$, otherwise $R$ is a Type-2 rectangle.

  Observe that Type-1 rectangles either have $\ell_A$ as the unique left blocker or have $r_A$ as the unique right blocker, or both. The rectangle that has both $\ell_A$ as the unique left blocker and $r_A$ as the unique right blocker is a top extension of $A$ and we call it the root of the rectangles in $\RR_A$.
  Whereas, Type-2 rectangles have both left and right blockers other than sides $\ell_A$ and $r_A$. In this case $R$ is a bottom extension of $R'$.
  

  From the inductive hypothesis, we know that the $G[\RR_B]$ forms a tree. We consider the vertices in $\RR_A$.
  For every Type-1 rectangle in $R \in \RR_A$, there exists a unique $R' \in \RR_B$ such that $R$ and $R'$ have the same top blocker and the same left (right) blocker. For Type-2 rectangles $R \in \RR_A$, $R$ and $R'$ have both the same left and right blockers, in which case we call $R$ to be an extension of $R'$.

  
  Without loss of generality, we assume that the top side $t_A$ of $A$ intersects $\dP'$. The left, right, and bottom sides of $A$ are referred as $\ell_A, r_A, b_A$ in the rest of the proof.
  
  We classify the rectangles in $\RR^K(P)$ that intersect the bottom side $b_A$ of $A$ as follows.
  \begin{enumerate}
  \item \emph{Type-1 rectangles.} The rectangles either have a unique left blocker which is $\ell_A$ or have a unique right blocker which is $r_A$, or both. The rectangle $R_C$ that has both $\ell_A$ as the unique left blocker and $r_A$ as the unique right blocker is called the center rectangle among the type-1 rectangles.
  \item \emph{Type-2 rectangles.} The rectangles that have both left and right blockers other than sides $\ell_A$ and $r_A$.
  \end{enumerate}

  For every type-1 rectangle $R \in \RR^K(P)$ there exists a rectangle in $R' \in \RR^K(P')$ such that $R$ and $R'$ have the same set of top blockers. Furthermore, if $R$ has a left-blocker $s$ (resp. right blockers) other than $\ell_A$ (resp. $r_A$) then $R'$ also has $s$ as a left-blocker (resp. right blocker). We say $R'$ is the image of $R$ and observe that from Lemma~\ref{lem:equi-blocked}, $R$ has a unique image.

  Also, observe that if $R$ is a type-2 rectangle then there exists $R' \in \RR^K(P')$ such that $R' = R\setminus A$. Hence, if there are no type-1 rectangles then the support graph for $(\RR^K(P'),\dP')$ is also the support graph for $(\RR^K(P), \dP)$.
  
  Given the drawing of support graph of $(\RR^K(P'), \dP')$ that has all vertices corresponding to rectangles intersecting $t_A$ on the outer face, we add a path consisting of the type-1 rectangles, with the ghost rectangle $R_C$  in the interior of the path.
  that both unique left and right blockers as $\ell_A$ and $r_A$, respectively, and the set of ghost rectangles from left to right with a decreasing order of their height until they meet $R_C$. Similarly, rectangles in increasing order of their heights from left to right. See figure...

  Next we detach the subtree rooted at $R' \in \RR^K(P')$ and attach it to $R \in \RR^K(P)$ where $R$ is a ghost rectangle and $R'$ is its image.
  
  
We claim that for every rectangle $R \in \RR^K(P)\setminus \RR^K(P')$ there exists a rectangle $R' \in \RR^K(P')$ such that $R$ and $R'$ share a corner. Furthermore, there exists a planar drawing of the support graph of $(\RR^K(P'), \dP')$ such that the set of the images of rectangles in $\RR^K(P) \setminus \RR^K(P')$ lie on the outer boundary of the support graph and they induce a path. We need to make a copy of the path and put an edge between $R$ and $R'$ where $R \in \RR^K(P)\setminus \RR^K(P')$ and $R'$ is its image in $\RR^K(P')$.
\end{proof}


\begin{definition}[Blocker of an Area-Maximal Rectangle]
Given an orthogonal polygon $P$ and an area-maximal rectangle $R \subseteq P$, any side $s$ of $P$ is called a blocker of $R$ if $s \cap \partial R \neq \emptyset$. If $s$ intersects the top (resp. bottom, left, right) side of $R$ then $s$ is called a top (resp. bottom, left, right) blocker of $R$.
\end{definition}

\begin{lemma}
  \label{lem:equi-blocked}
Given an orthogonal polygon $P$, and two area-maximal rectangles $R$ and $R'$ in $P$, if $R$ and $R'$ have the same set of top, left, and right blockers then $R=R'$.
\end{lemma}


\begin{definition}[Vertically Blocked Rectangles]
  Given an orthogonal polygon $P$, an area-maximal rectangle $R \subseteq P$ is called vertically blocked if there exists vertical line $\ell_v$, a top blocker $t \in \dP$ and a bottom blocker $b \in \dP$ of $R$ such that $\ell_v \cap t \neq \emptyset$ and $\ell_v \cap b \neq \emptyset$.
\end{definition}

\begin{lemma}
  {\label{lem:opp-blockers}}
  Given a simple orthogonal polygon, no $2$ distinct area-maximal rectangles have the same blockers in the opposite directions, viz., top and bottom or left and right.
\end{lemma}

\begin{proof}
  For the sake of contradiction, assume that there exists a simple orthogonal polygon $P$, and $2$ distinct area-maximal rectangles $A$ and $B$ that have the same blockers on their top and bottom direction. Consider the left sides of $A$ and $B$.
  Either their left sides are distinct or same. If they are distinct then one of the left side is to the left side of the other rectangle.  Let $A$'s left side be to the left of $B$'s left side. This means $B$'s left blocker is contained in $A$, which contradicts the fact that $A$ is an area-maximal rectangle.
  The other case is when their left side are same. Then one argues the same for their right sides. If their right sides are distinct then one can argue similarly as above and lead to a contradiction. If the right sides are also same then the $A$ and $B$ are the same rectangle.
\end{proof}


\begin{lemma}
Given a simple orthogonal polygon, if $2$ area-maximal rectangles have the set of their common blockers exactly in $2$ adjacent directions, viz., top and left, left and bottom, bottom and right, or right and top. Then the two rectangles are distinct.
\end{lemma}

\begin{proof}
  Suppose the two rectangles are not distinct. Then the set of common blockers is in all the $4$ directions.
\end{proof}

\begin{definition}
We say $R$ is a top (resp. bottom, left, right) extension of $R'$ if $R$ can be obtained by scaling $R'$ in the top (viz., bottom, left, right) direction.
\end{definition}


\begin{lemma}[Edge Support]
  Given a simple orthogonal polygon $P$, and a set of area-maximal rectangles $\RR$ such that for every $R \in \RR$ has a segment $s \in \dP$ as their bottom (resp. top, left, and right) blocker. Then the support graph on the hypergraph $(\RR,s)$ is a forest.
\end{lemma}

\begin{proof}
  The horizontal projections of the rectangles in $\RR$ forms a set of intervals. Moreover, we claim that the set of intervals forms a laminar family i.e., if two such distinct intervals $R_X:= [a,b]$ and $R_x':= [c,d]$ intersect then either $R_x \subset R_x'$ or  $R_x' \subset R_x$. Suppose otherwise is true, and without loss of generality, we assume, $a < c < b < d$. Then left blocker of $\RR_x'$ is contained in $\RR_x$, which is a contradiction.

  For every laminar family of intervals one can define a forest, where we have a node for every interval and $R_x'$ is a descendent of $R_x$ if $R_x' \subset R_x$.
\end{proof}

Moreover, observe that the support graph of $(\RR,s)$ is a tree, if the intersection graph of $\RR$ is connected.

\begin{lemma}
  $G$ is a support graph of $(\RR^K(P), \dP)$. 
\end{lemma}

\begin{proof}
  From the inductive hypothesis, we know that $G'$ is a support graph of $(\RR^K(P'), \dP')$. There are the following cases:
  \begin{enumerate}
  \item $A_x \subset B_x$.
  \item $B_x \subset A_x$. Attach $B$ to $A$.
  \item $A_x \setminus B_x \neq \emptyset$ and $B_x \setminus A_x \neq \emptyset$. There are at most $2$ Type-1 rectangles in $\RR_A$, i.e., $A$ and possibly the other rectangle whose only left (resp. right) blocker is $\ell_A$ (resp. $r_A$).

    There are possibly 2 rectangles such that 
    
  \end{enumerate}
  
\end{proof}

\begin{lemma}
  $G$ is planar.
\end{lemma}

\begin{lemma}
  For every leaf $v \in T(P)$, the vertices corresponding to the rectangles in $T(P)$ are on the outer face of $G$.
\end{lemma}




==> sections/proof-induction-v1.tex <==
\section{Existence of Planar Boundary Supports}

We shall denote the set of all area-maximal rectangles in a simple orthogonal polygon $P$ by $\RR^K(P)$. We will first prove two easy cases and then use them to prove the main theorem.

\begin{theorem}
  \label{thm:main}
  Given a simple orthogonal polygon $P$ and a set of area maximal rectangles $\RR$ with respect to $P$, there exists planar support graphs for $(\RR,\dP)$.
\end{theorem}

\begin{definition}[Star family]
  A family of rectangles $\RR$ and a polygon $P$ are said to be a star family if the following holds:
  \begin{enumerate}
  \item $\RR = \{R_1,\dots, R_t, R_c\}$ where if $R_i \cap R_j \neq \emptyset$ then $R_i \cap R_j \subseteq R_c$, for $1 \le i < j \le t$. We refer $R_c$ as the center rectangle of the star family.
  \item Every rectangle in $\RR$ is area-maximal with respect to $P$.
  \end{enumerate}
\end{definition}

See Figure so-and-so for an example of a star family.

\begin{lemma}
Every star family has a boundary support that is a star graph.
\end{lemma}

\begin{lemma}
  \label{lem:etoile-sans-centre}
Every star family without its center rectangle, i.e. $(\RR\setminus R_c, \dP))$, has a planar support.
\end{lemma}

\begin{lemma}
  \label{lem:hereditary-planar}
  Given a simple orthogonal polygon $P$ and a set of area-maximal rectangles $\RR$ with respect to $P$. If $(\RR,\dP)$ has a planar support then for every $\RR' \subset \RR$, $(\RR',\dP)$ also has a planar support.
\end{lemma}

\begin{proof}
  We borrow the ideas of the left-right planarity test, attributed to de Fraysseix, Rosenstiehl, and de Mendez \cite{}.
  A finite graph $G$ is planar iff there exists a $F$-coloring of the cotree edges with respect to a depth-first-tree $T$ on $G$.
  If for every $v \in V$ and outgoing edges $e_i$ and $e_j$ from $v$, the following two condition are satisfied.
  \begin{itemize}
  \item
    All return edges of $e_i$ ending strictly higher than $lowpt(e_j)$ belong to one class, and
  \item
    All return edges of $e_j$ ending strictly higher than $lowpt(e_i)$ belong to the other class.
  \end{itemize}

  We are given a planar support graph $G$ for $(\RR,\dP)$. We claim that for every $R \in \RR$, there exists a planar support graph $G'$ for $(\RR\setminus\{R\},\dP)$.

  Consider a DFS tree $T$ defined on $G$ rooted at $v_R$. As $G$ is planar there exists a left-right coloring of the cotree edges. For all the cotree edges $(x_{i,j},v)$ that points from $x_{i,j}$ and return to $v$, where $x_{i,j}$ is in a subtree rooted at $w_i$, where $w_i$ is a child of $v$ in $T$. We replace the edge $(x_{i,j}, v)$ by $(x_{i,j}, w_i)$ retaining the color class of this new cotree edge. We call this replacement operation \emph{shortcutting}.

  For every $p \in dP$, if $\RR_p$ lies in some subtree rooted at $w_i$, for some $i \in [t]$, then $\RR_p$ is supported by this shortcutting. If $\RR_p$ is distributed across subtrees rooted at multiple children of $v$ then we claim that we can connect the vertices $\{w_i | i \in [t]\}$ such that $\RR_p$ is supported. Note we can ignore the descendants of $w_i$, for every $i \in [t]$ and only consider the children of $v$ in order to support $\RR_p$.

  \begin{enumerate}
  \item $\cup_{i \in [t]}R(w_i) \subset P$. Let $P' := \cup_{i \in [t]}R(w_i)$. $P'$ has complexity strictly smaller than $P$. We inductively argue that  $(\cup_{i \in [t]}R(w_i), \dP')$ has a planar support.
    
  \item $\cup_{i \in [t]}R(w_i) = P$.
    This precisely an instance of star family without the center rectangle. In our case, the center rectangle is $R(v)$. From Lemma~\ref{lem:etoile-sans-centre}, $(\cup_{i \in [t]} R(w_i), \dP)$ has a planar support. For every distict $i, j \in [t]$ the vertices in the subtrees rooted at $w_i$ and $w_j$ are independent, hence the subtrees can be independently drawn.
    
  \end{enumerate}
  
  Let this new graph be called $G'$.

  It is obvious, that the cotree edges in $G'$ have an $F$-coloring, thus $G'$ is planar.

  What remains to be proven is that $G'$ is a support graph for $(\RR\setminus\{R\}, \dP)$. To that end, consider a point $p \in \dP$. We claim that $G[\RR_p\setminus\{R\}]$ is connected. If $R \notin \RR_p$ there is nothing to prove.
  We assume that $R \in \RR_p$ without loss of generality and $\RR_p$ contains at least one other rectangle other than $R$. Also, note that the vertices corresponding to $\RR_p$ lies only in a subtree rooted at one of the children of $v$. 
\end{proof}



%%% Some definitions and lemmata %%%
\begin{definition}[Blocker of an Area-Maximal Rectangle]
Given an orthogonal polygon $P$ and an area-maximal rectangle $R \subseteq P$, any side $s$ of $P$ is called a blocker of $R$ if $s \cap \partial R \neq \emptyset$. If $s$ intersects the top (resp. bottom, left, right) side of $R$ then $s$ is called a top (resp. bottom, left, right) blocker of $R$.
\end{definition}

\begin{lemma}
  \label{lem:equi-blocked}
Given an orthogonal polygon $P$, and two area-maximal rectangles $R$ and $R'$ in $P$, if $R$ and $R'$ have the same set of top, left, and right blockers then $R=R'$.
\end{lemma}


\begin{definition}[Vertically Blocked Rectangles]
  Given an orthogonal polygon $P$, an area-maximal rectangle $R \subseteq P$ is called vertically blocked if there exists vertical line $\ell_v$, a top blocker $t \in \dP$ and a bottom blocker $b \in \dP$ of $R$ such that $\ell_v \cap t \neq \emptyset$ and $\ell_v \cap b \neq \emptyset$.
\end{definition}

\begin{lemma}
  {\label{lem:opp-blockers}}
  Given a simple orthogonal polygon, no $2$ distinct area-maximal rectangles have the same blockers in the opposite directions, viz., top and bottom or left and right.
\end{lemma}

\begin{proof}
  For the sake of contradiction, assume that there exists a simple orthogonal polygon $P$, and $2$ distinct area-maximal rectangles $A$ and $B$ that have the same blockers on their top and bottom direction. Consider the left sides of $A$ and $B$.
  Either their left sides are distinct or same. If they are distinct then one of the left side is to the left side of the other rectangle.  Let $A$'s left side be to the left of $B$'s left side. This means $B$'s left blocker is contained in $A$, which contradicts the fact that $A$ is an area-maximal rectangle.
  The other case is when their left side are same. Then one argues the same for their right sides. If their right sides are distinct then one can argue similarly as above and lead to a contradiction. If the right sides are also same then the $A$ and $B$ are the same rectangle.
\end{proof}


\begin{lemma}
Given a simple orthogonal polygon, if $2$ area-maximal rectangles have the set of their common blockers exactly in $2$ adjacent directions, viz., top and left, left and bottom, bottom and right, or right and top. Then the two rectangles are distinct.
\end{lemma}

\begin{proof}
  Suppose the two rectangles are not distinct. Then the set of common blockers is in all the $4$ directions.
\end{proof}

\begin{definition}
We say $R$ is a top (resp. bottom, left, right) extension of $R'$ if $R$ can be obtained by scaling $R'$ in the top (viz., bottom, left, right) direction.
\end{definition}


\begin{lemma}[Forest Support on Segments]
  \label{lem:laminar}
  Given a simple orthogonal polygon $P$, and a set of area-maximal rectangles $\RR$ such that for every $R \in \RR$, their bottom (resp. top, left, and right) blocker exists on a segment $s \in \dP$. Then there exists a support graph on the hypergraph $(\RR,s)$ that is a forest.
\end{lemma}

\begin{proof}
  The horizontal projections of the rectangles in $\RR$ forms a set of intervals. Moreover, we claim that the set of intervals forms a laminar family i.e., if two such distinct intervals $R_X:= [a,b]$ and $R_x':= [c,d]$ intersect then either $R_x \subset R_x'$ or  $R_x' \subset R_x$. Suppose otherwise is true, and without loss of generality, we assume, $a < c < b < d$. Then left blocker of $\RR_x'$ is contained in $\RR_x$, which is a contradiction.

  For every laminar family of intervals one can define a forest, where we have a node for every interval and $R_x'$ is a descendent of $R_x$ if $R_x' \subset R_x$.
\end{proof}

Moreover, observe that the forest support graph of $(\RR,s)$ is a tree, if the intersection graph of the intervals that are obtained by projecting the rectangles in $\RR$ on $s$ is connected.

%%% %%% 


\begin{definition}[Horizontal R-Tree \cite{}]
  Given a simple orthogonal polygon $P$, we horizontally cut $P$ along all its concave corners. This partitions $P$ into a set of interior disjoint rectangles $R_1,\uplus\dots,\uplus R_m$. We define a graph $T(P) = (V_T,E_T)$ where we have a vertex $v_i$ corresponding to $R_i$, for every $1\le i \le m$, and $(v_i,v_j) \in E_T$ if $\partial R_i \cap \partial R_j \neq \emptyset$.
\end{definition}

\begin{lemma}
Given a simple orthogonal polygon $P$, $T(P)$ is a tree.
\end{lemma}


%\begin{definition}[Complexity of an Orthogonal Polygon]
%  Given an orthogonal polygon $P$, the complexity of $P$ is the number of corners $P$ has including both convex and concave corners. We shall refer this qauntity by $|P|$.
%\end{definition}



Let $v$ be a leaf in $T(P)$. Then $\RR_v$ be the set of rectangles whose bottom blocker is the bottom side of $v$.
Invariants: 
\begin{enumerate}
  \item
    $G[\RR_v]$ is a tree.
  \item
    If $v$ is a leaf of $T(P)$ then $\RR_v$ appears on the outer face of the plane graph $G$.
\end{enumerate}

  

\begin{lemma}
  Given a simple orthogonal polygon $P$ and let $\RR^K(P)$ be the set of all area-maximal rectangles with respect to $P$.
   $(\RR^K(P),\dP)$ has a planar support. Furthermore, there is a plane graph of the support such that the vertices corresponding to the vertically-blocked rectangles of $P$ are in its outer face.
\end{lemma}

\begin{proof}

  We consider $T(P)$, the horizontal R-Tree of $P$. We prove inductively on the number of vertices of $T(P)$.
  The base case is when there is a single vertex in $T(P)$, i.e., $P$ is a rectangle and the claim of the lemma is trivially true.
  
  Let $A \subset P$ be rectangle that corresponds to a leaf of $T(P)$.
  Let $P' := P \setminus A$. Also let $B$ be the parent of $A$ in $T(P)$.
  The inductive case is that, if the statement of the lemma is true for $P'$ then it is also true for $P$. Thus, the inductive hypothesis is that the lemma holds true for $P'$.

  The high-level idea is to attach the vertices of $\RR_A$ to some of the vertices of $\RR_{B}$ and also remove some of the subtrees at $\RR_B$ and attach it to vertices in $\RR_A$.

  As every rectangle $R \in\RR_A$ has the bottom side of $A$ as its bottom blocker, therefore from Lemma~\ref{lem:opp-blockers}, $R$ can be uniquely determined by its top blocker $t_R$. Similarly, every rectangle in $\RR_B$ can be uniquely determined by its top blocker.

  If $A_x \subset B_x$ then for every $R \in \RR_A$, there exists a unique $R' \in \RR_B$ such that $R$ and $R'$ have a common top blocker. We say $R'$ is an image of $R$.

  Otherwise, when $B_x \subset A_x$, then for every $R' \in \RR_B$ there exists a unique $R \in \RR_A$ such that $R$ and $R'$ have a common top blocker, i.e., $t_R = t_{R'}$. We again say $R'$ is an image of $R$. Observe that  $v_A$ is the only vertex in $\RR_A$ that has no image in $\RR_B$ because the top blocker of $v_A$ is $t_A$ and none of the vertices in $\RR_B$ has $t_A$ as their top blocker. corresponding to the rectangle $A$. We will assume that $A_x \subset B_x$ for the rest of the proof. At the end we will show that for the other case we only need to add edges to $v_A$ 

  There are two cases: given $R \in \RR_A$ either $R'\in \RR^K(P)$ or not.
  We say $R \in \RR_A$ is a Type-1 rectangle if $R' \in \RR^K(P)$, otherwise $R$ is a Type-2 rectangle.

  Observe that Type-1 rectangles either have $\ell_A$ as the unique left blocker or have $r_A$ as the unique right blocker, or both. The rectangle that has both $\ell_A$ as the unique left blocker and $r_A$ as the unique right blocker is a top extension of $A$ and we call it the root of the rectangles in $\RR_A$.
  Whereas, Type-2 rectangles have both left and right blockers other than sides $\ell_A$ and $r_A$. In this case $R$ is a bottom extension of $R'$.
  

  From the inductive hypothesis, we know that the $G[\RR_B]$ forms a tree. We consider the vertices in $\RR_A$.
 % For every Type-1 rectangle in $R \in \RR_A$, there exists a unique $R' \in \RR_B$ such that $R$ and $R'$ have the same top blocker and the same left (right) blocker. For Type-2 rectangles $R \in \RR_A$, $R$ and $R'$ have both the same left and right blockers, in which case we call $R$ to be an extension of $R'$.

  
  Without loss of generality, we assume that the top side $t_A$ of $A$ intersects $\dP'$. The left, right, and bottom sides of $A$ are referred as $\ell_A, r_A, b_A$ in the rest of the proof.
  
  Given the drawing of support graph of $(\RR^K(P'), \dP')$ that has all vertices corresponding to rectangles intersecting $t_A$ on the outer face, we add a path consisting of the type-1 rectangles, with the ghost rectangle $R_C$  in the interior of the path.
  that both unique left and right blockers as $\ell_A$ and $r_A$, respectively, and the set of ghost rectangles from left to right with a decreasing order of their height until they meet $R_C$. Similarly, rectangles in increasing order of their heights from left to right. See figure...

  Next we detach the subtree rooted at $R' \in \RR^K(P')$ and attach it to $R \in \RR^K(P)$ where $R$ is a ghost rectangle and $R'$ is its image.
  
  
  We claim that for every rectangle $R \in \RR^K(P)\setminus \RR^K(P')$ there exists a rectangle $R' \in \RR^K(P')$ such that $R$ and $R'$ share a corner. Furthermore, there exists a planar drawing of the support graph of $(\RR^K(P'), \dP')$ such that the set of the images of rectangles in $\RR^K(P) \setminus \RR^K(P')$ lie on the outer boundary of the support graph and they induce a path. We need to make a copy of the path and put an edge between $R$ and $R'$ where $R \in \RR^K(P)\setminus \RR^K(P')$ and $R'$ is its image in $\RR^K(P')$.

  \begin{lemma}
    For every planar support graph $G$ of $(\RR^K(P), b_B \cap t_A)$ there exists a planar support graph $H$ of $(\RR^K(P), b_A)$, such that $G$ is an induced subgraph of $H$.
  \end{lemma}

  \begin{proof}
    Consider the following cases:
     \begin{enumerate}
  \item \textbf{$A_x \subset B_x$.} In this case the horizontal projections of $b_B \cap t_A$ and $b_A$ are the same. Hence, a support graph of $(\RR^K(P), b_B \cap t_A)$ is also a support graph of $(\RR^K(P), b_A)$.
  \item \textbf{$A_x \setminus B_x \neq \emptyset$.} From Lemma~\ref{lem:laminar}, we know that there exists a rooted tree support graph $G$ of $(\RR^K(P), b_B \cap t_A)$. Attaching the vertex $v_A$, corresponding to rectangle $A$, to the root of $G$ is a valid support graph of $(\RR^K(P), b_A)$. Also, planarity is preserved as $v_A$ is a degree-1 vertex.
     \end{enumerate}
     
  \end{proof}
  
  
  \begin{lemma}
    If $A_x \subset B_X$ then there exists support graphs $G$ of $(\RR^K(P'), b_B \cap t_A)$ and $H$ of $(\RR^K(P), b_B \cap t_A)$, such that $G$ and $H$ are isomorphic to each other.
    If $A_x \setminus B_x \neq \emptyset$ then there exists 
  \end{lemma}

  \begin{lemma}
    \label{lem:path-supp}
There exists support graphs of $(\RR_A^{(1)}, b_A)$ that are path graphs, where $\RR_A^{(1)}$ is the set of Type-1 vertices in $\RR_A$.
  \end{lemma}

  \begin{proof}
Observe that the set $\RR^{(1)}_A$ can be grouped into two subsets where one subset contains the Type-1 rectangles whose unique left blocker is $l_A$ and the other subset contains those whose unique right blocker is $r_A$. There may exist a top extension of $A$ in both these subsets. Thus, we can order the rectangles from left to right such that the rectangles in the first subset appears before those in the second subset, with the top extension of $A$ in between. Among the first group we order the rectangles based on their relative distance of their right sides from $\ell_A$, with the one whose right side is closest to $\ell_A$ appears first in this ordering. Conversely, we order the rectangles in the second group based on their relative distance of their left sides from $r_A$, with the one whose left side is closest to $r_A$ appears last in the ordering. See Figure ...
  \end{proof}
  

  \begin{lemma}
    If $A_x \subset B_x$ then there exists a tree support graph $G$ of $(\RR_A, b_A)$ and tree support graph $H$ of $(\RR_B, b_B)$ such that $G$ is isomorphic to a subgraph of $H$.
  \end{lemma}


  \begin{lemma}
    If $B_x \subset A_x$ then there exists a tree support graph $G$ of $(\RR_A, b_A)$ and tree support graph $H$ of $(\RR_B, b_B)$ such that $H$ is isomorphic to a subgraph of $G$.
  \end{lemma}

  \begin{proof}
Observe that every vertex in $\RR_A$ except $v_A$, has an image in $\RR_B$. Moreover, if there exists $R_i, R_j \in \RR_A$ such that $R_i <_p R_j$ then  $R_i' <_p R_j'$ where $R_i', R_j' \in \RR_B$ are images of $R_i$ and $R_j$, respectively. Thus, the tree structure defined on $\RR_B$ due to the partial order $<_p$ is isomorphic to the tree structure defined on $\RR_A \setminus \{v_A\}$.
  \end{proof}
  
  \begin{lemma}
    Given $B_x \subset A_x$, if there exists a planar support $G_{P'}$ for $(\RR^K(P'), \dP')$ then there exists a planar support $G_P$ for $(\RR^K(P), \dP)$.
  \end{lemma}
  \begin{proof}
Consider $G_{P'}$ and attach vertex $v_A$ by adding the edge $(v_A, v_B)$. We also relabel the vertices of $\RR_B$, for every $R' \in \RR_B$, we relabel it to $R \in \RR_A$. The resultant graph is also planar as $v_A$ has degree $1$. 
  \end{proof}
  
  %%% Algorithm to draw G_P from G_P' %%%
  
  \subsubsection*{From $G_{P'}$ to $G_P$.}
  Observe, $\RR^K(P) = (\RR^K(P') \cup \RR_A)\setminus f(\RR^{(2)}_A)$, where $f(\RR^{(2)}_A) := \{f(R) \in \RR_B \mid R \in \RR^{(2)}_A \}$.
  Given a planar drawing of $G_{P'}$ with the invariant ***.
  \begin{algorithm}
    \caption{Algorithm to draw planar support inductively}
    \label{alg:draw}  
    \begin{algorithmic}[1]

    %\textbf{Input:} $G_P' = (\RR^K(P'), E)$\;

    %\textbf{Output:} $G_P = (\RR^K(P), E)$\;
      
    %\item
    \If{$B_x \subset A_x$}

    \State $E \gets E \cup \{(A,B^{\uparrow})\}$\;

    % \ref{proc:rename}\;
    
    % \State $\forall R_i \in \RR^{(2)}_A$, \textbf{rename} $f(R_i)$ to $R_i$\;

    \ForAll{$R_i \in \RR^{(2)}_A$}
    
    \State \textbf{rename} $f(R_i)$ to $R_i$\;
    
    \EndFor

    %\State {return $G_P = (\RR^K(P), E)$}\;
    
    \State \Return $G_P = (\RR^K(P), E)$\;
     
    \EndIf
    
\If{$\RR^{(1)}_A \neq \emptyset$}

    \State $i \gets 1$\;

    \While{$i < |\RR^{(1)}_A|$}
    
    \State $E \gets E \cup \{(R_i, R_{i+1})\}$\; %% as defined by the natural ordering on $\RR^{(1)}_A$, as defined in the proof of Lemma~\ref{lem:path-supp},
    \label{alg:type1-path}

    \State $E \gets E \cup \{(R_i, f(R_i))\}$\;
    \label{alg:type1-image}
    
        \State $i \gets i + 1$\;
    
    \EndWhile

    \State $E \gets E \cup \{(R_i, f(R_i))\}$\;
      
    %\item  
      %Furthermore, for every Type-1 vertex $R \in \RR^{(1)}_A$, we put an edge $(R,f(R))$.
    %\item

    %\Else %goto Step~\ref{it:T2}.

      %\State $\forall R_i \in \RR^{(2)}_A$, \textbf{rename} $f(R_i)$ to $R_i$\;
    \ForAll{$R_i \in \RR^{(2)}_A$}
    
    \State \textbf{rename} $f(R_i)$ to $R_i$\;
    
    \EndFor
     % \State \textbf{return $G_P = (\RR^K(P), E)$}\;

\State \Return $G_P = (\RR^K(P), E)$\;
     
\EndIf

\If{$\RR^{(2)}_A \neq \emptyset$}

    \ForAll{$(R_i,R_j) \in \TT(\RR_A)$  where $R_i$ is the parent of $R_j$ in $\TT(\RR_A)$, $R_j \in \RR^{(2)}_A$ and $R_i \in \RR^{(1)}_A$}

    \State $E \gets E \setminus \{(f(R_i), f(R_j))\}$\;
    \label{alg:del}
    \State $E \gets E \cup \{(R_i,f(R_j))\}$\;
    \label{alg:add}

    \EndFor

      %\label{proc:rename}
      %\State $\forall R_i \in \RR^{(2)}_A$, \textbf{rename} $f(R_i)$ to $R_i$\;
    \ForAll{$R_i \in \RR^{(2)}_A$}
      
        \State \textbf{rename} $f(R_i)$ to $R_i$\;
    \EndFor
      \EndIf
      
   %\State \textbf{return $G_P = (\RR^K(P), E)$}\;
      
\State \Return $G_P = (\RR^K(P), E)$\;
%      \label{it:T2}

\end{algorithmic}
\end{algorithm}
  
\end{proof}

%%% End of the proof to the complete family.


\begin{lemma}
  $G$ is a support graph of $(\RR^K(P), \dP)$. 
\end{lemma}

\begin{proof}
  From the inductive hypothesis, we know that $G_{P'}$ is a support graph of $(\RR^K(P'), \dP')$. There are the following cases:
  \begin{enumerate}[label=\textbf{Case \arabic*:}]
  \item $B_x \subset A_x$.

    $E(G_{P'}) \cup \{(A,B^\uparrow)\}$ ensures that every point in $A\cap \dP$ is supported.
    
  \item $A_x \subset B_x$.

    As $G_{P'}$ is a support graph for $(\RR^K(P'), \dP')$, we only need to ensure that all points in the set
    $\{R \cap \dP \mid R \in \RR_A \}$ are supported by $G_{P}$. Note that $\{R \cap \dP \mid R \in \RR_A \}$ is the set of all blockers of every $R \in \RR_A$. Also, recall that $b_A$ is the set of all bottom blockers of $R \in \RR_A$. Further observe that all the edges in $\TT(\RR_A)$ are included in $G_P$. This is because, edges between two Type-1 vertices are added in Step~\ref{alg:type1-path}, edges between Type-1 and Type-2 vertices are added in Step~\ref{alg:add}, and edges between two Type-2 vertices are present as their images in $\RR_B$ are renamed, in Algorithm~\ref{alg:draw}.
    Hence, $b_A$ is supported by $G_P$.

    Next, we claim that all the top blockers of $R \in \RR_A$ are also supported. If $R$ is a Type-1 vertex then the top blocker is supported because the edge $(R,f(R))$ is added in Step~\ref{alg:type1-image}. If furthermore, $R$ is the top extension of $A$, then one or two reflex vertices of $P$ incident with the corners of $A$. In that case, those reflex vertices are also supported by $(A^{\uparrow}, f(A^{\uparrow}))$.
    If $R$ is a Type-2 vertex then its top blocker is satisfied once $f(R)$ is relabeled as $R$ in $G_{P}$ as the top blocker of $f(R)$ was satisfied in $G_{P'}$.

    Finally, we claim that all the left and right blockers of $R \in \RR_A$ are also supported by $G_P$. If $R$ is a Type-2 vertex then its left and right blockers are satisfied for the same reason as above. If $R$ is a Type-1 vertex and it is also the top extension of $A$, then its left blocker is $\ell_A$ and its right blocker is $r_A$. Then $\ell_A$ is satisfied by all Type-1 vertices to the left of $R$ in the path of the Type-1 vertices and $r_A$ is satisfied by all the Type-2 vertices to the right of $R$ in that path. This path is formed iteratively by Step~\ref{alg:type1-path} of the algorithm. If $R$ is a Type-1 vertex whose left blocker is not $\ell_A$, then such a left blocker is satisfied by the edge $(R,f(R))$, which is added at Step~\ref{alg:type1-image} of the algorithm.


    %\item $A_x \setminus B_x \neq \emptyset$ and $B_x \setminus A_x \neq \emptyset$. There are at most $2$ Type-1 rectangles in $\RR_A$, i.e., $A$ and possibly the other rectangle whose only left (resp. right) blocker is $\ell_A$ (resp. $r_A$).
   % There are possibly 2 rectangles such that 
    
  \end{enumerate}
  
\end{proof}


\begin{lemma}
  \label{lem:neigh-tree}
For every $R_i, R_j \in \RR_B$, $N(R_i) \cap N(R_j) \neq \emptyset$ where $N(X)$ is the neighborhood of $X$ in $G_{P'}\setminus \RR_B$.
\end{lemma}

\begin{proof}
  As $R_i, R_j \in \RR_B$, there respective bottom blockers lie on $b_B$. For the sake of contradiction, assume that there exists $R_k \notin \RR_B$ such that $(R_k,R_i), (R_k,R_j) \in E(G_{P'})$.
  \begin{enumerate}
  \item
    $R_i \cap R_j \neq \emptyset$. This means either one of them pierces the other, i.e., $R_i <_f R_j$ or $R_j <_f R_i$. We can always keep the adjacnecy with the fatter rectangle and remove the edge with the thinner rectangle keeping the support property satisfied.
  \item
    $R_i \cap R_j = \emptyset$. This means that there exists a rectangle $R_{\ell} \in \RR_B$ such that $R_i, R_j <_f R_{\ell}$ and $R_i \cap R_k \subseteq R_{\ell}$ and $R_j \cap R_k \subseteq R_\ell$. Thus, having $(R_k,R_\ell)$ instead of $(R_k,R_i)$ and $(R_k,R_j)$ is enough to satisfy the support property. It is also not too difficult to see that introducing $(R_k,R_\ell)$, if it was not present, and removing the other two vertices does not create any crossings, as $R_\ell$ is an ancestor of $R_i$ and $R_j$ in $\TT(\RR_B)$.
  \end{enumerate}
\end{proof}


\begin{lemma}
  $G_P$ is planar.
\end{lemma}

\begin{proof}
  %For every leaf $v \in T(P)$, the vertices corresponding to the rectangles in $T(P)$ are on the outer face of $G$.


  It is trivial that planarity is preserved at the end of Step 1 of Algorithm 1.
  The left to right ordering of the Type-1 vertices $(R_i, \dots, R_j)$ along the path is same as that $(f(R_i), \dots, f(R_j))$.
  Thus, the edges at Step 2 can also be drawn without crossing any edges.
  From Lemma~\ref{lem:neigh-tree}, the neighbours of Type-2 vertices are trees, hence planarity is ensured by the cut-paste operation at Step 3 of Algorithm 1.

  If $B_x \subset A_x$ then $G_P$ is planar because a single edge $(A^{\uparrow}, B^{\uparrow})$ is added to $G_{P'}$.

  Let $A_x \subset B_x$.
  If $\RR^{(1)}_A \neq \emptyset$ then edges $(R_i, R_{i+1})$, for $i < |\RR^{(1)}_A|$ can be drawn without crossing as they form a path.
  Also note, the edges $(R_i, f(R_i))$, for $R_i \in \RR^{(1)}_A$ can also be drawn without crossing, because the vertices $f(R_i)$'s are drawn on the outer face of $G_{P'}$, and if $R_i <_1 R_j$ then $f(R_i) <_1 f(R_j)$. See figure ...

  If $\RR^{(2)}_A \neq \emptyset$ and Steps~\ref{alg:del} and \ref{alg:add} of Algorithm \ref{alg:draw} are executed, then from Lemma~\ref{lem:neigh-tree} planarity is ensured.
\end{proof}


\subsection*{Assumption.} We assume that given a simple orthogonal polygon $P$ every area-maximal rectangle in $P$ has positive horizontal and vertical lengths. If $P$ is such that there exists a rectangle with zero horizontal/vertical length, we can always do transformation preserving the number of area-maximal rectangles in $P$. This assumption is made for the ease of exposition.





==> sections/proof-induction.tex <==
\section{Existence of Planar Boundary Supports}

We shall denote the set of all area-maximal rectangles in a simple orthogonal polygon $P$ by $\RR^K(P)$. We will first prove two special cases (Theorem~\ref{thm:complete-rect} and Lemma~\ref{lem:hereditary-planar}) and then use them to prove the following main theorem.

\begin{theorem}
  \label{thm:main}
  Given a simple orthogonal polygon $P$ and a set of area maximal rectangles $\RR$ with respect to $P$, there exists planar support graph for $(\RR,\dP)$.
\end{theorem}

\begin{proof}
  From Theorem~\ref{thm:complete-rect} it follows that $(\RR^K(P), \dP)$ has a planar support. By repeatedly applying Lemma~\ref{lem:hereditary-planar} we prove that $(\RR, \dP)$ has a planar support, as $\RR \subseteq \RR^K(P)$.
\end{proof}
 
Before we prove Lemma~\ref{lem:hereditary-planar}, we state a definition and a few lemmata.

\begin{definition}[Star family]
  A family of area-maximal rectangles $\RR = \{R_1,\dots, R_t, R_c\}$ with respect to a simple orthogonal polygon $P$ is said to be a star family, if the following holds:
  if there exists $p \in \dP$ such that $R_i, R_j \in \RR_p$ then $R_c \in \RR_p$, for $1 \le i < j \le t$. We refer $R_c$ as the center rectangle of the star family.
\end{definition}

See Figure so-and-so for an example of a star family.

\begin{lemma}
Every star family has a boundary support that is a star graph.
\end{lemma}

\begin{lemma}
Given a corner $p$ of $R_c$, there exists at most one $R_i \in \RR$ such that $R_i$ and $R_c$ have a corner intersection and $R_i$ contains $p$.
\end{lemma}

Thus, there are at most $4$ rectangles in $\RR$ with whom $R_c$ has a corner intersection, each containing exactly one of its corners.

  From Definition~\ref{defn:pierce-poset}, we can partition the star family without its center into the following subsets. The set of rectangles that have a corner intersection with $R_c$ that we denote by $\RR_N$. The rectangles that have a piercing intersection with $R_c$. Furthermore, we call the rectangles $R \in \RR$ to be vertical rectangles if $R \prec R_c$, i.e., $\RR_V := \{R \in \RR \mid R \prec R_c\}$. Likewise, we call the rectangles $R \in \RR$ to be horizontal rectangles if $R_c \prec R$, i.e., $\RR_H := \{R \in \RR \mid R_c \prec R \}$. Observe that as every rectangle in $\RR \setminus \{R_c\}$ has a non-empty intersection with $R_c$, they belong to one of these three subsets, i.e., $\RR := \RR_N \uplus \RR_V \uplus \RR_H \uplus \{R_c\}$.

  We define the subset of maximal vertical rectangles with respect to the the poset $\prec$ as $\RR^*_V := \max\{R \in \RR_V\}$. Similarly, we define the subset of minimal horizontal rectangles $\RR^*_H := \min\{R \in \RR_H\}$.

  \begin{lemma}
    Given a corner $p$ of $R_c$, there exists at most one rectangle $R \in \RR$ that contains $p$ in its interior.
  \end{lemma}

  \begin{proof}
  \end{proof}
  
  \begin{lemma}
There does not exist $3$ rectangles in $\RR^*_V$ (resp. $\RR^*_H$) such that each one has a corner intersection with the other two.
  \end{lemma}

  \begin{proof}

  \end{proof}

  \begin{definition}
    Define a linear ordering $<_v$ on the rectangles in $\RR^*_V$, such that $R <_v R'$ if the left side of $R$ is to the left of that of $R'$, for every $R, R' \in \RR^*_V$.
  \end{definition}

  Let $\RR^*_V = \{V_1, \dots, V_k\}$, where $V_1 <_v \dots <_v V_k$.

  \begin{definition}
    Define a linear ordering $<_h$ on the rectangles in $\RR^*_H$, such that $R <_h R'$ if the bottom side of $R$ is below that of $R'$, for every $R, R' \in \RR^*_H$.
  \end{definition}
      
  Let $\RR^*_H = \{H_1, \dots, H_\ell\}$, where $H_1 <_h \dots <_h H_\ell$.
  
%  We prove by induction on the size of the set $\RR$. Observe that every rectangle $R \in \RR \setminus R_c$ is of the following type. Either $R$ intersects two adjacent sides of $R_c$ or it intersects the two opposite sides of $R_c$. If it of the former type, then there can be at most $4$ of them as $R_c$ has $4$ corners, and we shall call them corner rectangles. If $R$ is of the latter type then it either intersects the two horizontal sides or the two vertical sides of $R_c$. If $R$ intersects the two horizontal (resp. vertical) sides then we call it a horizontal (resp. vertical) rectangle. Observe that two horizontal (resp. vertical) rectangles are disjoint. \why
%  Also observe that a corner rectangle, can intersect at most 1 vertical (resp., horizontal) rectangle.

  % Let $V_1, \dots, V_k$ be the horizontal rectangles in $\RR \setminus R_c$ where $V_1$ is the leftmost and $V_k$ is the rightmost rectangle. Similarly, let $H_1, \dots, H_\ell$ be the horizontal rectangles in $(\RR\setminus R_c, \dP)$ where $H_1$ is the topmost and $H_\ell$ is the bottommost rectangle.
  We refer $V_1, V_k, H_1,$ and $H_\ell$ to be terminal rectangles.

  If $V_1$ and $R_c$ have a common left blocker, then we call $V_1$ to be left-aligned. Likewise, if $V_k$ and $R_c$ have a common right blocker, then we call $V_k$ to be right-aligned. Conversely, if $H_1$ and $R_c$ have a common top blocker, then we call $H_1$ to be top-aligned. Finally, if $H_\ell$ and $R_c$ have a common bottom blocker, then we call $H_\ell$ to be bottom-aligned. Note that the terminal rectangles may or may not be aligned.

  \subsubsection{Algorithm to draw planar support for a center-less star family}
  In the following we give a simple algorithm to draw a planar support of $(\RR\setminus R_c, \dP)$.
  We put an edge between the left-aligned (resp.~right-aligned) rectangle, if it exists, and every horizontal rectangle. Similarly, we put an edge between the top-aligned (resp.~bottom-aligned) rectangle, if it exists and every vertical rectangle. Without loss of generality, assume that all the aligned rectangles exist. Then define a cycle $C_4$ on $\{V_1, H_1, V_k, H_\ell\}$ with edges alternating between the horizontal and vertical rectangles. We place the vertices corresponding to the other horizontal rectangles $H_j$, in the inner face of the $C_4$ and draw edges $(V_1,H_j)$ and $(V_k,H_j)$, for $1 < j < \ell$. Conversely, place the vertices corresponding to the other vertical rectangles $V_i$ in the outer face of the $C_4$ and draw edges $(V_i, H_1)$ and $(V_i, H_k)$, for $1 < i < k$. If there exists corner rectangle intersecting a terminal rectangle, then we put an edge between them. See Figure so-and-so.

  \begin{lemma}
  \label{lem:etoile-sans-centre}
Every star family without its center rectangle, i.e. $(\RR\setminus R_c, \dP))$, has a planar support.
\end{lemma}

\begin{proof}

  It is easy to see that the resultant graph is planar. It is also a support graph because if $R_i \cap R_j \cap \dP \neq \emptyset$ then we have an edge $(R_i, R_j)$ in our graph, for every $R_i, R_j \in \RR\setminus \{R_c\}$. From Observation~\ref{obs:int-supp}, an intersection graph is a support graph with respect to an intersecting family of sets.
\end{proof}

\begin{lemma}
  \label{lem:hereditary-planar}
  Given a simple orthogonal polygon $P$ and a set of area-maximal rectangles $\RR$ with respect to $P$. If $(\RR,\dP)$ has a planar support then for every $\RR' \subset \RR$, $(\RR',\dP)$ also has a planar support.
\end{lemma}

\begin{proof}
  We borrow the ideas of the left-right planarity test, attributed to de Fraysseix, Rosenstiehl, and de Mendez \cite{}.
  A finite graph $G$ is planar iff there exists a $F$-coloring of the cotree edges with respect to a depth-first-tree $T$ on $G$.
  If for every $v \in V$ and outgoing edges $e_i$ and $e_j$ from $v$, the following two condition are satisfied.
  \begin{itemize}
  \item
    All return edges of $e_i$ ending strictly higher than $lowpt(e_j)$ belong to one class, and
  \item
    All return edges of $e_j$ ending strictly higher than $lowpt(e_i)$ belong to the other class.
  \end{itemize}

  We are given a planar support graph $G$ for $(\RR,\dP)$. We claim that for every $R \in \RR$, there exists a planar support graph $G'$ for $(\RR\setminus\{R\},\dP)$.

  Consider a DFS tree $T$ defined on $G$ rooted at $v_R$. As $G$ is planar there exists a left-right coloring of the cotree edges. For all the cotree edges $(x_{i,j},v)$ that points from $x_{i,j}$ and return to $v$, where $x_{i,j}$ is in a subtree rooted at $w_i$, where $w_i$ is a child of $v$ in $T$. We replace the edge $(x_{i,j}, v)$ by $(x_{i,j}, w_i)$ retaining the color class of this new cotree edge. We call this replacement operation \emph{shortcutting}. % and say that $G'$ is obtained by shortcutting $G$ at $v$.

  For every $p \in \dP$, if $\RR_p$ lies in some subtree rooted at $w_i$, for some $i \in [t]$, then $\RR_p$ is supported by this shortcutting. If $\RR_p$ is distributed across subtrees rooted at multiple children of $v$ then note the following observation.
  \begin{observation}
    If there exists vertices $x,y \in \RR_p$ such that $x \in T(w_i)$ and $y \in T(w_j)$, for $i,j \in [t]$ and $i \neq j$, then $w_i, w_j \in \RR_p$.
  \end{observation}

  This is true because otherwise point $p$ is not supported by $G$.
  Therefore, we can ignore the descendants of $w_i$, for every $i \in [t]$ and only put edges among the $w_i$'s in order to support $\RR_p$.

  We claim that $\{w_1, \dots, w_t, v\}$ forms a star family where $v$ is the center of the star.
  \begin{enumerate}
  \item $\cup_{i \in [t]}R(w_i) \subset P$. Let $P' := \cup_{i \in [t]}R(w_i)$. $P'$ has complexity strictly smaller than $P$. We inductively argue that  $(\{ R(w_i) \mid i \in [t]\}, \dP')$ has a planar support.
    
  \item $\cup_{i \in [t]}R(w_i) = P$.
    This is precisely an instance of star family without the center rectangle. \why
    In our case, the center rectangle is $R(v)$. From Lemma~\ref{lem:etoile-sans-centre}, $(\cup_{i \in [t]} R(w_i), \dP)$ has a planar support. For every distinct $i, j \in [t]$ the vertices in the subtrees rooted at $w_i$ and $w_j$ are independent, hence the subtrees can be independently drawn.
    
  \end{enumerate}
  
  Let this new graph be called $G'$.

  It is obvious, that the cotree edges in $G'$ have an $F$-coloring, thus $G'$ is planar.

  What remains to be proven is that $G'$ is a support graph for $(\RR\setminus\{R\}, \dP)$. To that end, consider a point $p \in \dP$. We claim that $G[\RR_p\setminus\{R\}]$ is connected. If $R \notin \RR_p$ there is nothing to prove.
  We assume that $R \in \RR_p$ without loss of generality and $\RR_p$ contains at least one other rectangle other than $R$. Also, note that the vertices corresponding to $\RR_p$ lies only in a subtree rooted at one of the children of $v$. 
\end{proof}

\section{Complete Family of Area-Maximal Rectangles}
  Given a simple orthogonal polygon $P$, let $\RR^K(P)$ be the set of all area-maximal rectangles with respect to $P$. In this section we prove Theorem~\ref{thm:complete-rect}, i.e., $(\RR^K(P), \dP)$ has a planar support. To this end we shall present a few definitions and lemmata.

%%% Some definitions and lemmata %%%
\begin{definition}[Blocker of an Area-Maximal Rectangle]
Given an orthogonal polygon $P$ and an area-maximal rectangle $R \subseteq P$, any side $s$ of $P$ is called a blocker of $R$ if $s \cap \partial R \neq \emptyset$. If $s$ intersects the top (resp. bottom, left, right) side of $R$ then $s$ is called a top (resp. bottom, left, right) blocker of $R$.
\end{definition}


\begin{definition}[Vertically Blocked Rectangles]
  Given an orthogonal polygon $P$, an area-maximal rectangle $R \subseteq P$ is called vertically blocked if $R$ has a top blocker $(x,y_1)$ and a bottom blocker $(x,y_2)$.% vertical line $\ell_v$, a top blocker $t \in \dP$ and a bottom blocker $b \in \dP$ of $R$ such that $\ell_v \cap t \neq \emptyset$ and $\ell_v \cap b \neq \emptyset$.
\end{definition}

\begin{lemma}
  {\label{lem:opp-blockers}}
  Given a simple orthogonal polygon, no $2$ distinct area-maximal rectangles have the same blockers in the opposite directions, viz., top and bottom or left and right.
\end{lemma}

\begin{proof}
  For the sake of contradiction, assume that there exists a simple orthogonal polygon $P$, and $2$ distinct area-maximal rectangles $A$ and $B$ that have the same blockers on their top and bottom direction. Consider the left sides of $A$ and $B$.
  Either their left sides are distinct or same. If they are distinct then one of the left side is to the left side of the other rectangle.  Let $A$'s left side be to the left of $B$'s left side. This means $B$'s left blocker is contained in $A$, which contradicts the fact that $A$ is an area-maximal rectangle.
  The other case is when their left side are same. Then one argues the same for their right sides. If their right sides are distinct then one can argue similarly as above and lead to a contradiction. If the right sides are also same then the $A$ and $B$ are the same rectangle.
\end{proof}


\begin{lemma}
Given a simple orthogonal polygon, if $2$ area-maximal rectangles have the set of their common blockers exactly in $2$ adjacent directions, viz., top and left, left and bottom, bottom and right, or right and top. Then the two rectangles are distinct.
\end{lemma}

\begin{proof}
  Suppose the two rectangles are not distinct. Then the set of common blockers is in all the $4$ directions.
\end{proof}

\begin{definition}[Extension of a Rectangle]
We say $R$ is a top (resp. bottom, left, right) extension of $R'$ with respect to a polygon $P$ if $R$ can be obtained by scaling $R'$ in the top (viz., bottom, left, right) direction and $R$ is area-maximal with respect to $P$.
\end{definition}


\begin{lemma}[Forest Support on Segments]
  \label{lem:laminar}
  Given a simple orthogonal polygon $P$, and a set of area-maximal rectangles $\RR$ such that for every $R \in \RR$, their bottom (resp. top, left, and right) blocker exists on a segment $s \in \dP$. Then there exists a support graph on the hypergraph $(\RR,s)$ that is a forest.
\end{lemma}

\begin{proof}
  The horizontal projections of the rectangles in $\RR$ forms a set of intervals. Moreover, we claim that the set of intervals forms a laminar family i.e., if two such distinct intervals $R_X:= [a,b]$ and $R_x':= [c,d]$ intersect then either $R_x \subset R_x'$ or  $R_x' \subset R_x$. Suppose otherwise is true, and without loss of generality, we assume, $a < c < b < d$. Then left blocker of $\RR_x'$ is contained in $\RR_x$, which is a contradiction.

  For every laminar family of intervals one can define a forest, where we have a node for every interval and $R_x'$ is a descendent of $R_x$ if $R_x' \subset R_x$.
\end{proof}

Moreover, observe that the forest support graph of $(\RR,s)$ is a tree, if the intersection graph of the intervals that are obtained by projecting the rectangles in $\RR$ on $s$ is connected.








%%% %%% 


\begin{definition}[Horizontal R-Tree \cite{}]
  Given a simple orthogonal polygon $P$, we horizontally cut $P$ along all its concave corners. This partitions $P$ into a set of interior disjoint rectangles $R_1,\uplus\dots,\uplus R_m$. We define a graph $T(P) = (V_T,E_T)$ where we have a vertex $v_i$ corresponding to $R_i$, for every $1\le i \le m$, and $(v_i,v_j) \in E_T$ if $\partial R_i \cap \partial R_j \neq \emptyset$.
\end{definition}

\begin{lemma}
Given a simple orthogonal polygon $P$, $T(P)$ is a tree.
\end{lemma}

\begin{lemma}
  \label{lem:struct}
  Let $P$ be a simple orthogonal polygon with $B$ be a leaf of $T(P)$. Furthermore, let $R, R' \in \RR^K(P) \setminus \RR_B$ and $G_P$ be a minimal support graph of $(\RR^K(P), \dP)$. If $(R,R') \in E(G_{P})$ then we call $(R,R')$ an auxillary edge.
  If we keep contracting all the auxillary edges then eventually the contracted vertex has a unique neighbor $R''$ such that $R'' \in \RR_B$.
\end{lemma}

\begin{proof}
For the sake of contradiction, assume that there exists a contracted vertex that has multiple neighbors in $\RR_B$.
This means there exists $R \in \RR^K(P') \setminus \RR_B$, such that $R$ is biconnected to some $R'' \in \RR_B$ in $G_P'[\RR^K(P') \setminus \RR_B]$. We claim that this implies that $P'$ has a hole.
\end{proof}

%\begin{definition}[Complexity of an Orthogonal Polygon]
%  Given an orthogonal polygon $P$, the complexity of $P$ is the number of corners $P$ has including both convex and concave corners. We shall refer this qauntity by $|P|$.
%\end{definition}



%Let $v$ be a leaf in $T(P)$. Then $\RR_v$ be the set of rectangles whose bottom blocker is the bottom side of $v$.
%Invariants: 
%\begin{enumerate}
%  \item
%    $G[\RR_v]$ is a tree.
%  \item
%    If $v$ is a leaf of $T(P)$ then $\RR_v$ appears on the outer face of the plane graph $G$.
%\end{enumerate}

  

\begin{theorem}
  \label{thm:complete-rect}
   $(\RR^K(P),\dP)$ has a planar support. Furthermore, there is a plane graph of the support such that the vertices corresponding to the vertically-blocked rectangles of $P$ are in its outer face.
\end{theorem}

\begin{proof}

  We consider $T(P)$, the horizontal R-Tree of $P$. We prove inductively on the number of vertices of $T(P)$.
  The base case is when there is a single vertex in $T(P)$, i.e., $P$ is a rectangle and the claim of the lemma is trivially true.
  
  Let $A \subset P$ be rectangle that corresponds to a leaf of $T(P)$.
  Let $P' := P \setminus A$. Also let $B$ be the parent of $A$ in $T(P)$.
  The inductive case is that, if the statement of the lemma is true for $P'$ then it is also true for $P$. Thus, the inductive hypothesis is that the lemma holds true for $P'$.

  As, the vertices of the support graphs are rectangles, we shall interchangeably use rectangles and vertices to denote the same, which would be clear from the context.

     Denote, $\RR_A$ be the set of area-maximal rectangles in $\RR^K(P)$ that have their bottom blockers in $b_A$. Likewise, let $\RR_B$ be the set of area-maximal rectangles in $\RR^K(P')$ that have their bottom blockers in $b_B$.
  The high-level idea is to attach the vertices of $\RR_A$ to some of the vertices of $\RR_{B}$ and also remove some of the subtrees at $\RR_B$ and attach it to vertices in $\RR_A$.

  As every rectangle $R \in\RR_A$ has the bottom side of $A$ as its bottom blocker, therefore from Lemma~\ref{lem:opp-blockers}, $R$ can be uniquely determined by its top blocker $t_R$. Similarly, every rectangle in $\RR_B$ can be uniquely determined by its top blocker.

  We define a function $f : \RR_A \setminus \{A\} \rightarrow \RR_B$, where for every $R \in \RR_A \setminus \{A\}$ there exists $f(R) \in \RR_B$ and $t \in \dP'$ such that $t$ is a top blocker of both $R$ and $f(R)$. We say $f(R)$ is the image of $R$.
  Also, observe that Lemma~\ref{lem:opp-blockers} implies that $f$ is an injective mapping.

  %If $A_x \subset B_x$ then for every $R \in \RR_A$, there exists a unique $R' \in \RR_B$ such that $R$ and $R'$ have a common top blocker. We say $R'$ is an image of $R$.

  %Otherwise, when $B_x \subset A_x$, then for every $R' \in \RR_B$ there exists a unique $R \in \RR_A$ such that $R$ and $R'$ have a common top blocker, i.e., $t_R = t_{R'}$. We again say $R'$ is an image of $R$.

  %Observe that if $B_x \subset A_x$ then $A$ is the only vertex in $\RR_A$ that has no image in $\RR_B$ because the top blocker of $A$ is $t_A$ and none of the vertices in $\RR_B$ has $t_A$ as their top blocker. Hence, the function $f(\cdot)$ is defined on $\RR_A \setminus \{A\}$.

  %We will assume that $A_x \subset B_x$ for the rest of the proof. At the end we will show that for the other case we only need to add edges to $v_A$ 

  There are two cases: given $R \in \RR_A \setminus \{A\}$ either $f(R)\in \RR^K(P)$ or not.
  We say $R \in \RR_A\setminus \{A\}$ is a Type-1 rectangle if $f(R) \in \RR^K(P)$, otherwise $R$ is a Type-2 rectangle. If $A \in \RR_A$, then $A$ is neither Type-1 nor Type-2 rectangle. Henceforth, we denote the set of Type-1 (resp. Type-2) rectangles as $\RR^{(1)}_A$ (resp. $\RR^{(2)}_A$).

  Observe that Type-1 rectangles either have $\ell_A$ as the unique left blocker or have $r_A$ as the unique right blocker, or both. The rectangle that has both $\ell_A$ as the unique left blocker and $r_A$ as the unique right blocker is $A^\uparrow$, the top extension of $A$, and we call it the root of the rectangles in $\TT(\RR_A)$.
  Whereas, Type-2 rectangles have both left and right blockers other than sides $\ell_A$ and $r_A$. Thus, for every $R \in \RR^{(2)}_A$, $R = f(R)^{\downarrow}$, the bottom extension of $f(R)$.
  

  From the inductive hypothesis, we know that the $G[\RR_B]$ forms a tree. We consider the vertices in $\RR_A$.
 % For every Type-1 rectangle in $R \in \RR_A$, there exists a unique $R' \in \RR_B$ such that $R$ and $R'$ have the same top blocker and the same left (right) blocker. For Type-2 rectangles $R \in \RR_A$, $R$ and $R'$ have both the same left and right blockers, in which case we call $R$ to be an extension of $R'$.

  
  Without loss of generality, we assume that the top side $t_A$ of $A$ intersects $\dP'$. The left, right, and bottom sides of $A$ are referred as $\ell_A, r_A, b_A$ in the rest of the proof.
  
%  Given the drawing of support graph of $(\RR^K(P'), \dP')$ that has all vertices corresponding to rectangles intersecting $t_A$ on the outer face, we add a path consisting of the type-1 rectangles, with the ghost rectangle $R_C$  in the interior of the path.
%  that both unique left and right blockers as $\ell_A$ and $r_A$, respectively, and the set of ghost rectangles from left to right with a decreasing order of their height until they meet $R_C$. Similarly, rectangles in increasing order of their heights from left to right. See figure...

%  Next we detach the subtree rooted at $R' \in \RR^K(P')$ and attach it to $R \in \RR^K(P)$ where $R$ is a ghost rectangle and $R'$ is its image.
  
  
%  We claim that for every rectangle $R \in \RR^K(P)\setminus \RR^K(P')$ there exists a rectangle $R' \in \RR^K(P')$ such that $R$ and $R'$ share a corner. Furthermore, there exists a planar drawing of the support graph of $(\RR^K(P'), \dP')$ such that the set of the images of rectangles in $\RR^K(P) \setminus \RR^K(P')$ lie on the outer boundary of the support graph and they induce a path. We need to make a copy of the path and put an edge between $R$ and $R'$ where $R \in \RR^K(P)\setminus \RR^K(P')$ and $R'$ is its image in $\RR^K(P')$.

  \begin{lemma}
    For every planar support graph $G$ of $(\RR^K(P), b_B \cap t_A)$ there exists a planar support graph $H$ of $(\RR^K(P), b_A)$, such that $G$ is an induced subgraph of $H$.
  \end{lemma}

  \begin{proof}
    Consider the following cases:
     \begin{enumerate}
  \item \textbf{$A_x \subset B_x$.} In this case the horizontal projections of $b_B \cap t_A$ and $b_A$ are the same. Hence, a support graph of $(\RR^K(P), b_B \cap t_A)$ is also a support graph of $(\RR^K(P), b_A)$.
  \item \textbf{$A_x \setminus B_x \neq \emptyset$.} From Lemma~\ref{lem:laminar}, we know that there exists a rooted tree support graph $G$ of $(\RR^K(P), b_B \cap t_A)$. Attaching the vertex $v_A$, corresponding to rectangle $A$, to the root of $G$ is a valid support graph of $(\RR^K(P), b_A)$. Also, planarity is preserved as $v_A$ is a degree-1 vertex.
     \end{enumerate}
     
  \end{proof}
  
  
  \begin{lemma}
    If $A_x \subset B_X$ then there exists support graphs $G$ of $(\RR^K(P'), b_B \cap t_A)$ and $H$ of $(\RR^K(P), b_B \cap t_A)$, such that $G$ and $H$ are isomorphic to each other.
    If $A_x \setminus B_x \neq \emptyset$ then there exists 
  \end{lemma}

  \begin{lemma}
    \label{lem:path-supp}
There exists support graphs of $(\RR_A^{(1)}, b_A)$ that are path graphs, where $\RR_A^{(1)}$ is the set of Type-1 vertices in $\RR_A$.
  \end{lemma}

  \begin{proof}
    If $\RR^{(1)}_A \neq \emptyset$ then it can be grouped into two subsets where one subset $L(\RR^{(1)}_A)$ contains the Type-1 rectangles whose unique left blocker is $l_A$ and the other subset $R(\RR^{(1)}_A)$ contains those whose unique right blocker is $r_A$. There exists $A^\uparrow$, the top extension of $A$, in both these subsets. Thus, we can order the rectangles from left to right, such that if $R_i \in L(\RR^{(1)}_A)$ and $R_j \in R(\RR^{(1)}_A)$ then $R_i <_1 R_j$, with the top extension of $A$ in between. For $R_i, R_j \in L(\RR^{(1)}_A)$, $R_i <_1 R_j$ if $r_{R_i} < r_{R_j}$.
    Thus the one whose right side is closest to $\ell_A$ appears first in this ordering $<_1$.
    Conversely, $R_i, R_j \in R(\RR^{(1)}_A)$, $R_i <_1 R_j$ if $l_{R_i} < l_{R_j}$. Thus the one whose left side is closest to $r_A$ appears last in the ordering $<_1$. See Figure ...

    We define the path $\PP$ on $\RR^{(1)}_A$ such that $R_i$ and $R_{i+1}$ are adjacent in $\PP$ if they are consecutive with respect to the linear ordering $<_1$. From Lemma~\ref{lem:laminar}, it follows that $\PP$ is a support graph of $(\RR_A^{(1)}, b_A)$.
  \end{proof}
  

  \begin{lemma}
    If $A_x \subset B_x$ then there exists a tree support graph $G$ of $(\RR_A, b_A)$ and tree support graph $H$ of $(\RR_B, b_B)$ such that $G$ is isomorphic to a subgraph of $H$.
  \end{lemma}


  \begin{lemma}
    If $B_x \subset A_x$ then there exists a tree support graph $G$ of $(\RR_A, b_A)$ and tree support graph $H$ of $(\RR_B, b_B)$ such that $H$ is isomorphic to a subgraph of $G$.
  \end{lemma}

  \begin{proof}
Observe that every vertex in $\RR_A$ except $v_A$, has an image in $\RR_B$. Moreover, if there exists $R_i, R_j \in \RR_A$ such that $R_i <_p R_j$ then  $R_i' <_p R_j'$ where $R_i', R_j' \in \RR_B$ are images of $R_i$ and $R_j$, respectively. Thus, the tree structure defined on $\RR_B$ due to the partial order $<_p$ is isomorphic to the tree structure defined on $\RR_A \setminus \{v_A\}$.
  \end{proof}
  
  \begin{lemma}
    Given $B_x \subset A_x$, if there exists a planar support $G_{P'}$ for $(\RR^K(P'), \dP')$ then there exists a planar support $G_P$ for $(\RR^K(P), \dP)$.
  \end{lemma}
  \begin{proof}
Consider $G_{P'}$ and attach vertex $v_A$ by adding the edge $(v_A, v_B)$. We also relabel the vertices of $\RR_B$, for every $R' \in \RR_B$, we relabel it to $R \in \RR_A$. The resultant graph is also planar as $v_A$ has degree $1$. 
  \end{proof}
  
  %%% Algorithm to draw G_P from G_P' %%%
  
  \subsubsection*{From $G_{P'}$ to $G_P$.}
  Observe, $\RR^K(P) = (\RR^K(P') \cup \RR_A)\setminus f(\RR^{(2)}_A)$, where $f(\RR^{(2)}_A) := \{f(R) \in \RR_B \mid R \in \RR^{(2)}_A \}$.
  Given a planar drawing of $G_{P'}$ with the invariant ***.
  \begin{algorithm}
    \caption{Algorithm to draw planar support inductively}
    \label{alg:draw}  
    \begin{algorithmic}[1]

    %\textbf{Input:} $G_P' = (\RR^K(P'), E)$\;

    %\textbf{Output:} $G_P = (\RR^K(P), E)$\;
      
    %\item
    \If{$B_x \subset A_x$}

    \State $E \gets E \cup \{(A,B^{\uparrow})\}$\;

    % \ref{proc:rename}\;
    
    % \State $\forall R_i \in \RR^{(2)}_A$, \textbf{rename} $f(R_i)$ to $R_i$\;

    \ForAll{$R_i \in \RR^{(2)}_A$}
    
    \State \textbf{rename} $f(R_i)$ to $R_i$\;
    
    \EndFor

    %\State {return $G_P = (\RR^K(P), E)$}\;
    
    \State \Return $G_P = (\RR^K(P), E)$\;
     
    \EndIf
    
\If{$\RR^{(1)}_A \neq \emptyset$}

    \State $i \gets 1$\;

    \While{$i < |\RR^{(1)}_A|$}
    
    \State $E \gets E \cup \{(R_i, R_{i+1})\}$\; %% as defined by the natural ordering on $\RR^{(1)}_A$, as defined in the proof of Lemma~\ref{lem:path-supp},
    \label{alg:type1-path}

    \State $E \gets E \cup \{(R_i, f(R_i))\}$\;
    \label{alg:type1-image}
    
        \State $i \gets i + 1$\;
    
    \EndWhile

    \State $E \gets E \cup \{(R_i, f(R_i))\}$\;
      
    %\item  
      %Furthermore, for every Type-1 vertex $R \in \RR^{(1)}_A$, we put an edge $(R,f(R))$.
    %\item

    %\Else %goto Step~\ref{it:T2}.

      %\State $\forall R_i \in \RR^{(2)}_A$, \textbf{rename} $f(R_i)$ to $R_i$\;
    \ForAll{$R_i \in \RR^{(2)}_A$}
    
    \State \textbf{rename} $f(R_i)$ to $R_i$\;
    
    \EndFor
     % \State \textbf{return $G_P = (\RR^K(P), E)$}\;

\State \Return $G_P = (\RR^K(P), E)$\;
     
\EndIf

\If{$\RR^{(2)}_A \neq \emptyset$}

    \ForAll{$(R_i,R_j) \in \TT(\RR_A)$  where $R_i$ is the parent of $R_j$ in $\TT(\RR_A)$, $R_j \in \RR^{(2)}_A$ and $R_i \in \RR^{(1)}_A$}

    \State $E \gets E \setminus \{(f(R_i), f(R_j))\}$\;
    \label{alg:del}
    \State $E \gets E \cup \{(R_i,f(R_j))\}$\;
    \label{alg:add}

    \EndFor

      %\label{proc:rename}
      %\State $\forall R_i \in \RR^{(2)}_A$, \textbf{rename} $f(R_i)$ to $R_i$\;
    \ForAll{$R_i \in \RR^{(2)}_A$}
      
        \State \textbf{rename} $f(R_i)$ to $R_i$\;
    \EndFor
      \EndIf
      
   %\State \textbf{return $G_P = (\RR^K(P), E)$}\;
      
\State \Return $G_P = (\RR^K(P), E)$\;
%      \label{it:T2}

\end{algorithmic}
\end{algorithm}

  From Lemmata~\ref{lem:comp-support} and~\ref{lem:comp-planar}, the proof follows.
\end{proof}

%%% End of the proof to the complete family.


\begin{lemma}
  \label{lem:comp-support}
  $G$ is a support graph of $(\RR^K(P), \dP)$. 
\end{lemma}

\begin{proof}
  From the inductive hypothesis, we know that $G_{P'}$ is a support graph of $(\RR^K(P'), \dP')$. There are the following cases:
  \begin{enumerate}[label=\textbf{Case \arabic*:}]
  \item $B_x \subset A_x$.

    $E(G_{P'}) \cup \{(A,B^\uparrow)\}$ ensures that every point in $A\cap \dP$ is supported.
    
  \item $A_x \subset B_x$.

    As $G_{P'}$ is a support graph for $(\RR^K(P'), \dP')$, we only need to ensure that all points in the set
    $\{R \cap \dP \mid R \in \RR_A \}$ are supported by $G_{P}$. Note that $\{R \cap \dP \mid R \in \RR_A \}$ is the set of all blockers of every $R \in \RR_A$. Also, recall that $b_A$ is the set of all bottom blockers of $R \in \RR_A$. Further observe that all the edges in $\TT(\RR_A)$ are included in $G_P$. This is because, edges between two Type-1 vertices are added in Step~\ref{alg:type1-path}, edges between Type-1 and Type-2 vertices are added in Step~\ref{alg:add}, and edges between two Type-2 vertices are present as their images in $\RR_B$ are renamed, in Algorithm~\ref{alg:draw}.
    Hence, $b_A$ is supported by $G_P$.

    Next, we claim that all the top blockers of $R \in \RR_A$ are also supported. If $R$ is a Type-1 vertex then the top blocker is supported because the edge $(R,f(R))$ is added in Step~\ref{alg:type1-image}. If furthermore, $R$ is the top extension of $A$, then one or two reflex vertices of $P$ incident with the corners of $A$. In that case, those reflex vertices are also supported by $(A^{\uparrow}, f(A^{\uparrow}))$.
    If $R$ is a Type-2 vertex then its top blocker is satisfied once $f(R)$ is relabeled as $R$ in $G_{P}$ as the top blocker of $f(R)$ was satisfied in $G_{P'}$.

    Finally, we claim that all the left and right blockers of $R \in \RR_A$ are also supported by $G_P$. If $R$ is a Type-2 vertex then its left and right blockers are satisfied for the same reason as above. If $R$ is a Type-1 vertex and it is also the top extension of $A$, i.e, $R =A^\uparrow$ then its left blocker is $\ell_A$ and its right blocker is $r_A$. Then $\ell_A$ is satisfied by all Type-1 vertices to the left of $A^\uparrow$ and including $A^\uparrow$ in the path $\PP$ of the Type-1 vertices (as described in the proof of Lemma~\ref{lem:path-supp}). Conversely, $r_A$ is satisfied by all the Type-1 vertices to the right of $A^\uparrow$ in $\PP$, including $A^\uparrow$. This path is formed iteratively by Step~\ref{alg:type1-path} of the algorithm. If $R$ is a Type-1 vertex whose left blocker is not $\ell_A$, then such a left blocker is satisfied by the edge $(R,f(R))$, which is added at Step~\ref{alg:type1-image} of the algorithm.


    %\item $A_x \setminus B_x \neq \emptyset$ and $B_x \setminus A_x \neq \emptyset$. There are at most $2$ Type-1 rectangles in $\RR_A$, i.e., $A$ and possibly the other rectangle whose only left (resp. right) blocker is $\ell_A$ (resp. $r_A$).
   % There are possibly 2 rectangles such that 
    
  \end{enumerate}
  
\end{proof}


%% \begin{lemma}
%%   \label{lem:neigh-tree}
%% For every $R_i, R_j \in \RR_B$, $N(R_i) \cap N(R_j) \neq \emptyset$ where $N(X)$ is the neighborhood of $X$ in $G_{P'}\setminus \RR_B$.
%% \end{lemma}

%% \begin{proof}
%%   As $R_i, R_j \in \RR_B$, there respective bottom blockers lie on $b_B$. For the sake of contradiction, assume that there exists $R_k \notin \RR_B$ such that $(R_k,R_i), (R_k,R_j) \in E(G_{P'})$.
%%   \begin{enumerate}
%%   \item
%%     $R_i \cap R_j \neq \emptyset$. This means either one of them pierces the other, i.e., $R_i <_f R_j$ or $R_j <_f R_i$. We can always keep the adjacnecy with the fatter rectangle and remove the edge with the thinner rectangle keeping the support property satisfied.
%%   \item
%%     $R_i \cap R_j = \emptyset$. This means that there exists a rectangle $R_{\ell} \in \RR_B$ such that $R_i, R_j <_f R_{\ell}$ and $R_i \cap R_k \subseteq R_{\ell}$ and $R_j \cap R_k \subseteq R_\ell$. Thus, having $(R_k,R_\ell)$ instead of $(R_k,R_i)$ and $(R_k,R_j)$ is enough to satisfy the support property. It is also not too difficult to see that introducing $(R_k,R_\ell)$, if it was not present, and removing the other two vertices does not create any crossings, as $R_\ell$ is an ancestor of $R_i$ and $R_j$ in $\TT(\RR_B)$.
%%   \end{enumerate}
%% \end{proof}


\begin{lemma}
  $G_P$ is planar.
  \label{lem:comp-planar}
\end{lemma}

\begin{proof}
  %For every leaf $v \in T(P)$, the vertices corresponding to the rectangles in $T(P)$ are on the outer face of $G$.


%  It is trivial that planarity is preserved at the end of Step 1 of Algorithm 1.
%  The left to right ordering of the Type-1 vertices $(R_i, \dots, R_j)$ along the path is same as that $(f(R_i), \dots, f(R_j))$.
%  Thus, the edges at Step 2 can also be drawn without crossing any edges.
%  From Lemma~\ref{lem:neigh-tree}, the neighbours of Type-2 vertices are trees, hence planarity is ensured by the cut-paste operation at Step 3 of Algorithm 1.

  If $B_x \subset A_x$ then $G_P$ is planar because a single edge $(A, B^{\uparrow})$ is added to $G_{P'}$.

  Let $A_x \subset B_x$.
  If $\RR^{(1)}_A \neq \emptyset$ then edges $(R_i, R_{i+1})$, for $i < |\RR^{(1)}_A|$ can be drawn without crossing as they form a path.
  Also note, the edges $(R_i, f(R_i))$, for $R_i \in \RR^{(1)}_A$ can also be drawn without crossing, because the vertices $f(R_i)$'s are drawn on the outer face of $G_{P'}$, and if $R_i <_1 R_j$ then $f(R_i) <_1 f(R_j)$. See figure ...

  If $\RR^{(2)}_A \neq \emptyset$ and Steps~\ref{alg:del} and \ref{alg:add} of Algorithm \ref{alg:draw} are executed, then from Lemma~\ref{lem:struct} planarity is ensured.
\end{proof}


\subsection*{Assumption.} We assume that given a simple orthogonal polygon $P$ every area-maximal rectangle in $P$ has positive horizontal and vertical lengths. If $P$ is such that there exists a rectangle with zero horizontal/vertical length, we can always do transformation preserving the number of area-maximal rectangles in $P$. This assumption is made for the ease of exposition.





==> sections/proof.tex <==


\section{Boundary support graph of the hypergraph on rectangles}

In this section we prove Theorem~\ref{thm:planar-support}. To that end, given $(\RR,\dP)$ we define an intermediate graph $H$ and prove that it is outerplanar. Then we perform a sequence of edge contractions and claim that this new graph $G$ is the support graph of $(\RR,\dP)$.

%\begin{definition}
%	For every rectangle $R_i$, we identify $t_i$ as the top segment of its boundary, $b_i$ as its bottom segment, $\ell_i$ as its left segment, and $r_i$ as its right segment.
%\end{definition}
%
%\begin{lemma}
%	\label{lem:nested}
%	Let $R_i$ and $R_j$ be two maximal rectangles having their left sides $\ell_i$ and $\ell_j$ lying on line $\ell$ in the polygon P. If $\ell_i \cap \ell_j \neq \emptyset$ then either $\ell_i \subset \ell_j$ or $\ell_j \subset \ell_i$.
%\end{lemma}

%\begin{proof}
%	%Let $\ell_i := [a_i,b_i]$ and $\ell_j := [a_j,b_j]$.
%
%	Suppose the contrary is true, i.e., $\ell_i \cap \ell_j \neq \emptyset$ and neither conains the other as a proper subset. %Without loss of generality, this means $a_i < a_j < b_i < b_j$.
%There are three possibilities: $r_i$ is to the left of $r_j$, $r_j$ is to the left of $r_i$, or both $r_i$ and $r_j$ lie on the same line. If $r_i$ is to the left of $r_j$ then the top side $t_i$ of $R_i$ is inside $R_j$, which in turn means $R_i$ is not maximal, and it could have been extended further in the top direction. The other two cases leads to similar contradictions.
%\end{proof}


\begin{theorem}
	\label{thm:planar-support}
	The hypergraph $(\RR, \dP)$ has a planar support graph.
\end{theorem}

%For every side $s_i$ of $\dP$ let $\RR_i := \{ R \in \RR \mid R\cap s_i \neq \emptyset\}$, the subset of rectangles in $\RR$ one of whose sides intersect $s_i$. Further, let $\JJ_i := \{ R\cap s_i | R \in \RR_i \}$ be the set of intervals on $s_i$ upon projecting those rectangles in $\RR_i$



\subsection{Definition of Graph $H$}

Choose some corner point $p_0$ in $\partial P$ arbitrarily and let this be the starting point of the sequence.  
We define a cyclic sequence of vertices based on how we encounter the rectangles along $\partial P$. Every vertex in $H$ corresponds to a unique rectangle $R \in \RR$. Thus, $V(H)$ can be partioned into equivalence classes where each class corresponds to a rectangle $R \in \RR$.

Note, the closed curve $\partial P$ is a closed sequence of orthogonal segments $s_1, \dots, s_n$. For every segment $s_i$ let $\RR_i := \{ R \in \RR \mid R\cap s_i \neq \emptyset\}$, be the subset of rectangles in $\RR$ one of whose sides intersect $s_i$. Further, let $\JJ_i := \{ R\cap s_i | R \in \RR_i \}$ be the set of intervals on $s_i$ upon projecting those rectangles in $\RR_i$.

%\begin{lemma}
%There are no two intervals $(a,b)$ and $(c,d)$ in $\JJ_i$, for every $i \in [n]$ such that $a < c < b < d$.
%\end{lemma}
%
%\begin{proof}
%	This is true because every rectangle in $\RR$ is area-maximal.
%\end{proof}

For every side $s_i \in \partial P$, we define a set of vertices in $H$ and a linear order on them. We say for $u,v \in V(H)$, $u <_{\dP} v$ if $u$ appears before $v$ when we start traversing from $p_0$ along $\dP$ in clockwise direction.

We assume that the polygon is drawn on an integer grid. For every orthogonal line $\ell$, we consider the set of sides in $P$ incident on $\ell$. Let they be $s^\ell_1, \dots, s^\ell_{k_\ell}$. We consider the set of rectangles, one of whose sides lie in $\ell$.

%For the set of intervals $\JJ_i$, we have a sense of left and right endpoints. On traversing whenever the endpoint of an interval $I_j$ is encountered we place an avatar of the corresponding rectangle $a_j$. If two or more intervals share their left (resp. right) endpoints, we consider the corresponding sides of the respective rectangles. 



If we traverse starting from one end to the other along $\ell$ and record the rectangles that we enter and exit in a sequence, we call it the pattern for $\ell$. 
For every side $s^\ell_i$, the linear order on its vertices (avatars of rectangles) should be a continuous subsequence of the pattern of $\ell$, such that the last avatar of $s^\ell_i$ and the first avatar of the $s^\ell_{i+1}$ should correspond to the same rectangle. Furthermore, if we remove the last avatars of all $s^\ell_i$, $1 \le i < k_\ell$ and concatenate the resultant sequences we get back the pattern of $\ell$.

    \begin{figure}[h]
        \centering
        \includegraphics[width=\textwidth]{img/rect-111}
        \caption{A subset of rectangles $\{R_1,\dots,R_6\} \subset \RR$ that have a common baseline $\ell$ which in turn contains multiple sides $\{s_1,\dots,s_7\}$ of $P$.}
        \label{fig:rect-order}
    \end{figure}
Consider the example drawn in Figure~\ref{fig:rect-order}. There are $6$ rectangles $R_1, \dots R_6$ and there are $7$ sides $s_1, \dots, s_7$ incident on a common baseline $\ell$. For every $s_j$, there is a set of rectangles whose base intersects $s_j$. 
In this example the pattern for $\ell$ is $12324215651$,
and the subsequences of $s_1, \dots, s_7$ are as follows:
$s_1: 1$, $s_2: 1232$, $s_3: 242$, $s_4: 21$, $s_5: 15$, $s_6: 561$, $s_7: 1$.

Thus, for every side $s_i$ of $P$ we get a sequence of avatars (vertices in H) $a^i_{1},\dots,a^i_{k_i}$ and we put an edge between consecutive vertices in such a sequence, thus they form a path in graph $H$. For two consecutive sides $s^{\dP}_i$ and $s^{\dP}_{i+1}$ along $\dP$, we put an edge between $a^i_{k_i}$ and $a^{i+1}_1$. Note that these two sides either define a convex corner or a concave corner.

So far, the only edges we have put is between consecutive avatars within a sequence corresponding to a side of $P$ or between the last and first avatars of consecutive sides along $\dP$. We refer the union of these edges as $E_{\dP}$.

For $R \in \RR$, consider the subsequence of avatars that correspond to $R$, $a^R_1, \dots, a^R_{k_R}$ in the increasing order along $\dP$. We put edges between consecutive avatars thus forming a path for every $R \in \RR$. We refer the union of these edges as $E_{\RR}$.

$H$ is defined on the set of the avatars and $E_{\dP} \cup E_{\RR}$ is its edge set.

\begin{obs}
	The vertices of $H$ forms a cyclic sequence $(a_0, \dots, a_{m-1})$ where $a_i \in \RR$.
\end{obs}

\begin{lemma}
	\label{lem:rect-pat}
For every pair of rectangles $R_1, R_2 \in \RR$ the following are true:
\begin{enumerate}
	\item
		If $R_1 \cap R_2 = \emptyset$, then they admit a $12$-pattern over $\dP$.
	\item
		If $R_1 \cap R_2 \neq \emptyset$,
			\begin{enumerate}
				\item
					$R_1$ contains exactly one corner of $R_2$, and also $R_2$ contains exactly one corner of $R_1$. Then they again admit a $12$-pattern over $\dP$.
				\item
					$R_1$ and $R_2$ cross each other. Then they admit a $1212$-pattern over $\dP$.
				\item
					One or two sides of $R_1$ and $R_2$ lie on the same orthogonal line. Then they admit $1212$-pattern over $\dP$.
			\end{enumerate}
\end{enumerate}
\end{lemma}

\begin{proof}
	See Figure~\ref{fig:types}.
	As the rectangles are area-maximal all four sides of the rectangle intersects $\dP$.  
	Cases 1, 2(a) and (b) are easy to see. 
	For case 2(c), there are some sides of $\dP$ which intersects both the rectangles where the definition of graph $H$ is being used to write the avatars of the rectangles. Nevertheless, the pattern for this subcase is $1212$.
    \begin{figure}[h]
        \centering
        \includegraphics[width=\textwidth]{img/types1}
        \caption{The different cases in which a pair of rectangles may (not) intersect and the $12$ or $1212$ patterns they admit in the cyclic sequence along $\dP$. The tiny squares on the boundary of the rectangles are the places where $\dP$ intersects the rectangles.}
        \label{fig:types}
    \end{figure}
\end{proof}

\begin{lemma}
	If $H$ has a $123123$-pattern then $H$ is not planar.
\end{lemma}

\begin{proof}
See Figure~\ref{fig:123123} and also note how such a subsequence can be realized.

    \begin{figure}[h]
        \centering
        \includegraphics[width=\textwidth]{img/123123}
        \caption{}
        \label{fig:123123}
    \end{figure}

\end{proof}

\subsubsection*{A slight detour.}
In order, to avoid such a $123123$ pattern in $\RR$ we tweak our local search solution a bit. Recall that $\RR$ is the union of local search and optimum solutions. Let $R_1, R_2, R_3$ be the three rectangles involved in creating such a $123123$-pattern as shown in Figure~\ref{fig:123123}. If all three of these rectangles are in one of the solution (local search or optimum solution) then we replace $R_1$ and $R_3$ by $R'_1$ and $R'_3$ (bottom-right in Figure~\ref{fig:123123}).
If one of the rectangle is in one solution and the other two are in the other solution.
If the optimum solution has $R_1$ and $R_3$ then replace them by $R'_1$ and $R'_3$ otherwise in all cases, add $R'_1$ and $R'_3$ to the local search solution and remove either or/both $R_1$ and $R_3$ from it. Thus, the size of the local search solution will go up by at most one, every time there is a tweak required to remove a $123123$-pattern. Let $L'$ be the modified local search solution. If still one can prove $|L'| \le |OPT|(1+\epsilon)$, then the same bound holds for the original local search solution. 

\begin{definition}
	We define a conflict graph $K$ on the edge set $E_{\RR}$ of $H$, where if $(a,c)$ and $(b,d)$ have an edge in $K$ if $a <_{\dP} b <_{\dP} c <_{\dP} d$ where $<_{\dP}$ is the ordering of avatars along $\dP$. 
\end{definition}

Therefore, if two edges in $E_{\RR}$ are adjacent in the conflict graph $K$, then both of them cannot be drawn through the interior (resp. exterior) of $\dP$.

\begin{lemma}
	$K$ is a bipartite graph.
\end{lemma}

\begin{proof}
	Observe that two edges in $E_{\RR}$ are in conflict (i.e., are adjacent in graph $K$) if the rectangles corresponding to avatars $a$ and $b$ admit a $1212$ pattern. From Lemma~\ref{lem:rect-pat} the rectangles belong to either of cases 2(a) or 2(b). Given any pair of rectangles that intersect in the way as described in 2(b), the rectangles can be slightly modified such that they intersect as described in 2(a). It is known that the intersection graph of rectangles where they intersect only in a crossing way is a bipartite graph. If graph $K$ has an odd cycle then so does this bipartite graph, which is a contradiction.
\end{proof}

\begin{lemma}
$H$ is an outerplanar graph.
\end{lemma}

\begin{proof}

The vertices of $H$ lie on the curve $\dP$. 
Observe that the two parts of the bipartite graph $K$ decides which edges in $E_{\RR}$ are to be drawn through the interior and which through the exterior. The edges in one part are required to be drawn through the interior of the curve $\dP$ and the edges in the other part are drawn through the exterior of $\dP$. Lastly, the edges in $E_{\dP}$ are drawn along the 

\end{proof}


Next we define a graph $G$ by contracting every edge in $E_{\RR}$ and further claim that $G$ is a planar supprt of $(\RR, \dP)$.


\begin{lemma}
	\label{lem:supp-planar}
	$G$ is a planar graph.
\end{lemma}

\begin{proof}
	As $G$ is obtained by doing a series of edge contractions in $H$, which is an outerplanar graph, $G$ is planar.
\end{proof}

\begin{lemma}
	\label{lem:support}
	$G$ is a support graph of $(\RR, \dP)$.
\end{lemma}

\begin{proof}
We need to prove that for every $p \in \dP$, $G[\RR_p]$ is connected. If $p$ is a non-corner point of $P$ and it belongs to some side $s^{\ell}_i$ of $\dP$ then we consider the sequence of avatars generated due to this side. If the avatars are a strict subset of $\RR_p$ then we keep looking for sides $s^{\ell}_{i-1}$ and $s^{\ell}_{i+1}$. We keep moving to the neighboring sides along the orthogonal $\ell$, unless the union of avatars is a superset of $\RR_p$. All the avatars generated by a side are connected by edges in $E_{\dP}$ and the last avatar of a side and the the first avatar of the next side correspond to the same rectangle, which means they are joined by an edge in $E_{\RR}$, which is subsequently contracted in $G$. 

If $p \in \dP$ is a corner point, this means it is at the intersection of two consecutive sides along $\dP$, hence the last avatar of one and the first avatar of the next are joined by an edge in $E_{\dP}$.

Thus $\RR_p$ is connected for every $p \in \dP$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:planar-support}]
	Lemmata~\ref{lem:supp-planar} and~\ref{lem:support} together implies the statement of the theorem.
\end{proof}


==> sections/star-v1.tex <==
\section{A Star Family of Rectangles}
\label{sec:star}
  
\begin{definition}[Star family]
  \label{def:star}
  A family of area-maximal rectangles $\RR = \{R_1,\dots, R_t, R_c\}$ with respect to a simple orthogonal polygon $P$ is said to be a star family, if the following conditions hold:
  \begin{enumerate}
  \item
    For every $i \in [t]$, there exists $p \in \dP$ such that $p \in R_i \cap R_c$.
  \item
    If there exists $p \in \dP$ such that $p \in R_i \cap R_j$ then $p \in R_c$, for $1 \le i < j \le t$.
    \end{enumerate}
   We refer $R_c$ as the center rectangle of the star family.
\end{definition}

See Figure so-and-so for an example of a star family.

Note that the center of a star family need not be unique. We shall refer the set of the center rectangles as the \emph{kernel} of the star family.

\begin{lemma}
Every star family has a boundary support that is a star graph.
\end{lemma}

%\begin{lemma}
%Given a corner $p$ of $R_c$, there exists at most one $R_i \in \RR$ such that $R_i$ and $R_c$ have a corner intersection and $R_i$ contains $p$.
%\end{lemma}

%Thus, there are at most $4$ rectangles in $\RR$ with whom $R_c$ has a corner intersection, each containing exactly one of its corners.

  From Definition~\ref{defn:pierce-poset}, we can partition the star family without its center into the following subsets. The set of rectangles that have a corner intersection with $R_c$ that we denote by $\RR_N$. The rectangles that have a piercing intersection with $R_c$. Furthermore, we call the rectangles $R \in \RR$ to be vertical rectangles if $R \prec R_c$, i.e., $\RR_V := \{R \in \RR \mid R \prec R_c\}$. Likewise, we call the rectangles $R \in \RR$ to be horizontal rectangles if $R_c \prec R$, i.e., $\RR_H := \{R \in \RR \mid R_c \prec R \}$. Observe that as every rectangle in $\RR \setminus \{R_c\}$ has a non-empty intersection with $R_c$, they belong to one of these three subsets, i.e., $\RR := \RR_N \uplus \RR_V \uplus \RR_H \uplus \{R_c\}$.

  We define the subset of maximally vertical rectangles with respect to the the poset $\prec$ as $\RR^*_V := \max\{R \in \RR_V\}$. Similarly, we define the subset of minimally horizontal rectangles $\RR^*_H := \min\{R \in \RR_H\}$.

  \begin{lemma}
    Given a corner $p$ of $R_c$, there exists at most one rectangle $R \in \RR$ that contains $p$ in its interior.
  \end{lemma}

  \begin{proof}
  \end{proof}
  
  \begin{lemma}
There does not exist $3$ rectangles in $\RR^*_V$ (resp. $\RR^*_H$) such that each one has a corner intersection with the other two.
  \end{lemma}

  \begin{proof}

  \end{proof}

  \begin{definition}
    Define a linear ordering $<_v$ on the rectangles in $\RR^*_V$, such that $R <_v R'$ if the left side of $R$ is to the left of that of $R'$, for every $R, R' \in \RR^*_V$.
  \end{definition}

  Let $\RR^*_V = \{V_1, \dots, V_k\}$, where $V_1 <_v \dots <_v V_k$.

  \begin{definition}
    Define a linear ordering $<_h$ on the rectangles in $\RR^*_H$, such that $R <_h R'$ if the bottom side of $R$ is below that of $R'$, for every $R, R' \in \RR^*_H$.
  \end{definition}
      
  Let $\RR^*_H = \{H_1, \dots, H_\ell\}$, where $H_1 <_h \dots <_h H_\ell$.
  
%  We prove by induction on the size of the set $\RR$. Observe that every rectangle $R \in \RR \setminus R_c$ is of the following type. Either $R$ intersects two adjacent sides of $R_c$ or it intersects the two opposite sides of $R_c$. If it of the former type, then there can be at most $4$ of them as $R_c$ has $4$ corners, and we shall call them corner rectangles. If $R$ is of the latter type then it either intersects the two horizontal sides or the two vertical sides of $R_c$. If $R$ intersects the two horizontal (resp. vertical) sides then we call it a horizontal (resp. vertical) rectangle. Observe that two horizontal (resp. vertical) rectangles are disjoint. \why
%  Also observe that a corner rectangle, can intersect at most 1 vertical (resp., horizontal) rectangle.

  % Let $V_1, \dots, V_k$ be the horizontal rectangles in $\RR \setminus R_c$ where $V_1$ is the leftmost and $V_k$ is the rightmost rectangle. Similarly, let $H_1, \dots, H_\ell$ be the horizontal rectangles in $(\RR\setminus R_c, \dP)$ where $H_1$ is the topmost and $H_\ell$ is the bottommost rectangle.
  We refer $V_1, V_k, H_1,$ and $H_\ell$ to be terminal rectangles.

  If $V_1$ and $R_c$ have a common left blocker, then we call $V_1$ to be left-aligned. Likewise, if $V_k$ and $R_c$ have a common right blocker, then we call $V_k$ to be right-aligned. Conversely, if $H_1$ and $R_c$ have a common top blocker, then we call $H_1$ to be top-aligned. Finally, if $H_\ell$ and $R_c$ have a common bottom blocker, then we call $H_\ell$ to be bottom-aligned. Note that a terminal rectangle may or may not be aligned.

  The corner rectangles, if any, containing the left-bottom corner, left-top corner, right-bottom corner, and right-top corner of $R_c$ are referred as $R_{11}, R_{1\ell}, R_{k1},$ and $R_{k\ell}$, respectively.

  \subsubsection{Algorithm to draw planar support for a center-less star family}
  In the following we give a simple algorithm to draw a planar support of $(\RR\setminus R_c, \dP)$.
  We put an edge between the left-aligned (resp.~right-aligned) rectangle, if it exists, and every horizontal rectangle. Similarly, we put an edge between the top-aligned (resp.~bottom-aligned) rectangle, if it exists and every vertical rectangle. Without loss of generality, assume that all the aligned rectangles exist. Then define a cycle $C_4$ on $\{V_1, H_1, V_k, H_\ell\}$ with edges alternating between the horizontal and vertical rectangles. We place the vertices corresponding to the other horizontal rectangles $H_j$, in the inner face of the $C_4$ and draw edges $(V_1,H_j)$ and $(V_k,H_j)$, for $1 < j < \ell$. Conversely, place the vertices corresponding to the other vertical rectangles $V_i$ in the outer face of the $C_4$ and draw edges $(V_i, H_1)$ and $(V_i, H_k)$, for $1 < i < k$. If there exists corner rectangle intersecting a terminal rectangle, then we put an edge between them. See Figure so-and-so.

  \begin{algorithm}
    \caption{Algorithm to draw planar support for a center-less star family}
    \label{alg:star}
    \begin{algorithmic}[1]
      \State Draw a circle $C$ on the plane.\;
      
      \State Draw the vertices corresponding to the terminal rectangles on $C$, in the order $V_1, H_1, V_k, H_\ell$. \;

      \State Draw the vertices corresponding to $V_2, \dots, V_{k-1}$ in the interior of $C$ along a line joining $V_1$ and $V_k$, respecting the linear ordering $<_v$. \;

      \State Draw the vertices corresponding to $H_2, \dots, H_{\ell -1}$ in the exterior of $C$ along some curved line joining $H_1$ and $H_\ell$, respecting the linear ordering $<_h$.\;

      \State Draw the vertex corresponding to $R_{11}$ on $C$ betweeen $V_1$ and $H_1$.
      \If{$V_1 \cap R_{11} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{11},V_1)$.\;
      \EndIf
      \If{$H_1 \cap R_{11} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{11},H_1)$.\;
      \EndIf
      
      \State Draw the vertex corresponding to $R_{1 \ell}$ on $C$ betweeen $V_1$ and $H_\ell$.
      \If{$V_1 \cap R_{1\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{1\ell},V_1)$.\;
      \EndIf
      \If{$H_\ell \cap R_{1\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{1\ell},H_\ell)$.\;
      \EndIf

      \State Draw the vertex corresponding to $R_{k1}$ on $C$ betweeen $V_k$ and $H_1$.
      \If{$V_k \cap R_{k1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k1},V_k)$.\;
      \EndIf
      \If{$H_1 \cap R_{k1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k1},H_1)$.\;
      \EndIf
      
      \State Draw the vertex corresponding to $R_{k \ell}$ on $C$ betweeen $V_k$ and $H_\ell$.
      \If{$V_k \cap R_{k\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k\ell},V_k)$.\;
      \EndIf
      \If{$H_\ell \cap R_{k\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k\ell},H_\ell)$.\;
      \EndIf
      
      
      \If{$V_1$ is left-aligned}
      \ForAll{$H_j \in \RR^*_H$}
      \State Draw an edge $(V_1, H_j)$.
      \EndFor
      \EndIf

      \If{$V_k$ is right-aligned}
      \ForAll{$H_j \in \RR^*_H$}
      \State Draw an edge $(V_k, H_j)$.
      \EndFor
      \EndIf

      \If{$H_1$ is top-aligned}
      \ForAll{$V_i \in \RR^*_V$}
      \State Draw an edge $(V_i, H_1)$.
      \EndFor
      \EndIf

      \If{$H_\ell$ is bottom-aligned}
      \ForAll{$V_i \in \RR^*_V$}
      \State Draw an edge $(V_i, H_\ell)$.
      \EndFor
      \EndIf

      \State $i \gets 1$\;
      \For{$i < k$}
      \If{$V_i \cap V_{i+1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(V_i, V_{i+1})$.\;
      \EndIf
      \State $i \gets i + 1$
      \EndFor

      \State $j \gets 1$\;
      \For{$j < \ell$}
      \If{$H_j \cap H_{j+1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(H_j, H_{j+1})$.\;
      \EndIf
      \State $j \gets j + 1$
      \EndFor
      
    \end{algorithmic}
  \end{algorithm}
  

  \begin{lemma}
  \label{lem:etoile-sans-centre}
Every star family without its center rectangle, i.e. $(\RR\setminus R_c, \dP))$, has a planar support.
\end{lemma}

\begin{proof}

  It is easy to see that the resultant graph is planar. It is also a support graph because if $R_i \cap R_j \cap \dP \neq \emptyset$ then we have an edge $(R_i, R_j)$ in our graph, for every $R_i, R_j \in \RR\setminus \{R_c\}$. From Observation~\ref{obs:int-supp}, an intersection graph is a support graph with respect to an intersecting family of sets.
\end{proof}



==> sections/star.tex <==
\section{Family of Rectangles with a Kernel}
\label{sec:star}

The main results of this section are Lemmata~\ref{lem:star-kernel} and \ref{lem:etoile-sans-centre}, which in turn are used to prove Lemma~\ref{lem:hereditary-planar} in Section~\ref{sec:hereditary}.
(Please see Section~\ref{sec:star-appendix} for missing details.)
In the following, we define a kernel of a rectangle family.
Informally, Lemma~\ref{lem:star-kernel} says that if a rectangle family has a star graph as its support, then the rectangle corresponding to the center of the star belongs to the kernel. Lemma~\ref{lem:etoile-sans-centre} states that a family of rectangles without its kernel still has a planar support.
%In order to prove the statement we define a kernel of a rectangle family and observe several of its properties.

\begin{definition}[Kernel of a Family]
  Given a family of area-maximal rectangles $\RR$ with respect to a simple polygon $P$, the kernel of $(\RR, \dP)$ is defined as follows.
  $$ker(\RR) := \displaystyle\bigcap_{\substack{p \in \dP \\ |\RR_p| \ge 2}} \RR_p$$
  where $\RR_p:= \{R \in \RR \mid p \in R\}$.
\end{definition}

A family $(\RR, \dP)$ with non-empty kernel $ker(\RR)$ is called \emph{proper} if for every $R \in \RR$ there exists $p \in \dP$ such that $ker(\RR) \cup \{R\} \subseteq \RR_p$. See Figure~\ref{fig:proper-kernel} for an example of a family that is not proper.

\begin{figure}[h]
        \centering
        \includegraphics[width=0.6\textwidth]{img/proper-non-empty-kernel}
        \caption{$(\{R_i, R_j, R_k, R_\ell, R_c\}, \dP)$ has a non-empty kernel $\{R_c\}$ but it is not proper. Whereas, $(\{R_i, R_j, R_c\}, \dP)$ is proper and has the same kernel. Note that $\dP$ is drawn with red lines.}
        \label{fig:proper-kernel}
\end{figure}



% \begin{definition}[Star family]
%   \label{def:star}
%   A family of area-maximal rectangles $\RR = \{R_1,\dots, R_t, R_c\}$ with respect to a simple orthogonal polygon $P$ is said to be a star family, if the following conditions hold:
%   \begin{enumerate}
%   \item
%     For every $i \in [t]$, there exists $p \in \dP$ such that $p \in R_i \cap R_c$.
%   \item
%     If there exists $p \in \dP$ such that $p \in R_i \cap R_j$ then $p \in R_c$, for $1 \le i < j \le t$.
%     \end{enumerate}
%    We refer $R_c$ as the center rectangle of the star family.
% \end{definition}

% See Figure so-and-so for an example of a star family.

% Note that the center of a star family need not be unique. We shall refer the set of the center rectangles as the \emph{kernel} of the star family.

\begin{observation}
  \label{lem:kernel-star}
  Every proper family with a non-empty kernel has a boundary support that is a star graph with a center vertex corresponding to a kernel rectangle. 
\end{observation}

In the following, we show that the converse is also true.

\begin{lemma}
  \label{lem:star-kernel}
Given a family of area-maximal rectangles $\RR$ with respect to a simple orthogonal polygon $P$. If there exists a minimal support graph $G$ of $(\RR, \dP)$ such that $G$ is a star graph then the rectangle corresponding to the center of $G$ belongs to $ker(\RR)$ and $\RR$ is proper.
\end{lemma}

\begin{proof}
  Let $R_c$ be the center of $G$. As $G$ is a minimal support graph of $(\RR, \dP)$, for every $p \in \dP$ such that $|\RR_p| \ge 2$, $R_c \in \RR_p$. If there exists $p \in \dP$ such that $|\RR_p| \ge 2$ and $R_c \notin \RR_p$ then $p$ is not supported by $G$ and hence a contradiction. This implies $R_c \in ker(\RR)$.

  $\RR$ is proper because otherwise there are isolated vertices in a minimal support. 
  %Consider the case where $(\RR,\dP)$ is a star family but its center $R_c$ does not correspond to the center of $G$.
  %Assume $(\RR, \dP)$ is not a star-family. Then either one or both the conditions in Definition~\ref{def:star} do not hold. If the first condition fails, i.e., if there exists a $R_i \in \RR$ such that $R_i \cap R_c \cap \dP = \emptyset$ then the edge $(R_i,R_c) \notin E(G)$ if $G$ is a minimal support. Hence, contradiction.
  %If the second condition fails, i.e., there exists $p \in \dP$ such that $p \in R_i \cap R_j$ and $p \notin R_c$. This implies $p$ is not supported in $G$ which is again a contradiction.
\end{proof}

%\begin{lemma}
%Given a corner $p$ of $R_c$, there exists at most one $R_i \in \RR$ such that $R_i$ and $R_c$ have a corner intersection and $R_i$ contains $p$.
%\end{lemma}

%Thus, there are at most $4$ rectangles in $\RR$ with whom $R_c$ has a corner intersection, each containing exactly one of its corners.

Throughout this section we assume $\RR$ to be proper and have a non-empty kernel. Without loss of generality, we consider $\RR$ to have a unique kernel rectangle, i.e., $ker(\RR) = \{R_c\}$.
From Definition~\ref{defn:pierce-poset}, we can partition the family without its kernel rectangle $R_c$ into the following subsets. The set of rectangles that have a corner intersection with $R_c$ that we denote by $\RR_N$. The remaining rectangles in $\RR$ have a piercing intersection with $R_c$. Among the ones having a piercing intersection, we call the rectangles $R \in \RR$ to be vertical rectangles if $R \prec R_c$, i.e., $\RR_V := \{R \in \RR \mid R \prec R_c\}$. Likewise, we call the rectangles $R \in \RR$ to be horizontal rectangles if $R_c \prec R$, i.e., $\RR_H := \{R \in \RR \mid R_c \prec R \}$.
%Observe that as every rectangle in $\RR \setminus \{R_c\}$ has a non-empty intersection with $R_c$, they belong to one of these three subsets, i.e.,
Thus, $\RR := \RR_N \uplus \RR_V \uplus \RR_H \uplus \{R_c\}$.

In the following, we are going to claim a few statements regarding how the rectangles from $\RR_N, \RR_V,$ and $\RR_H$ intersect among themselves.

\subsection{Corner Rectangles}

\begin{restatable}[$\star$]{lemma}{Corner}
%\begin{lemma}
  \label{lem:corner}
   Let $N \in \RR_N$ such that it contains the top-right corner of $R_c$. If there exists $R \in \RR$ such that $R \cap N \cap \dP \neq \emptyset$, then $R$ is either top-aligned and/or right-aligned with $R_c$.
   % \end{lemma}
   \end{restatable}
%   See~\ref{pr:corner}


   
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
\hide{ %appendix  
  \begin{proof}
    Given $N$ is a corner rectangle, there exists two points $p$ and $q$ where $\partial N \cap \partial R_c \neq \emptyset$. See Figure~\ref{fig:corner}.
    As $N \in \RR$ and $\RR$ is proper, at least one or both $p$ and $q$ belongs to $\dP$.
    If there exists $R \in \RR\setminus\{R_c\}$ such that $R \cap N \cap R_c \cap \dP \neq \emptyset$ then either $p$ or $q$ or both are contained in $R$. Without loss of generality, assume that $p \in R\cap \dP$. Then observe that the top side of $R$ is aligned with the top side of $R_c$. The left side of $R$ cannot be aligned with the left side of $N$, because otherwise there exists a point $p' \in \dP$ such that $p' \in (N \cap R \cap \dP)\setminus R_c$, which implies $R_c$ is not a kernel rectangle. See Figure~\ref{fig:corner}.
    Similarly, if $q \in R \cap \dP$ then the right side of $R$ is aligned with the right side of $R_c$.
    %This implies that $R$ cannot be a corner rectangle. For the same reason, $R$ cannot be a non-aligned vertical or horizontal rectangle.
  \end{proof}

}%hide

%\begin{restatable}{figure}{figcorner}
 \begin{figure}
        \centering
        \includegraphics[width=0.5\textwidth]{img/corner-vertical}
        \caption{Let $\RR$ be a proper family with $R_c$ as the kernel rectangle. The above figure shows parts of $\dP$ in bold red. Corner intersection $N \cap R_c \cap \dP = \{p,q\}$. If $R_j$ belongs to $\RR$ then $p'$ witnesses the intersection $N \cap R_j \cap \dP$ but it is outside $R_c$, which implies $R_c$ is not a kernel. However, $R_i$ can be part of $\RR$ without contradicting the fact that $R_c$ is the kernel rectangle.}
        \label{fig:corner}
       \end{figure}
 %     \end{restatable}
      
   \begin{hproof}
     See Figure~\ref{fig:corner} for an example.
   \end{hproof}
   
The following observation can be made from Lemma~\ref{lem:corner}.
\begin{observation}
  \label{lem:corner-disjoint}
    For $R_i, R_j \in \RR_N$, $R_i \cap R_j \cap \dP = \emptyset$.
  \end{observation}

%  The corner rectangles, if any, containing the bottom-left corner, top-left corner, top-right corner, and right-bottom corner of $R_c$ are referred as $N_{\swarrow}, N_{\nwarrow}, N_{\nearrow},$ and $N_{\searrow}$, respectively.
  
 \begin{restatable}[$\star$]{lemma}{CornerPattern}
% \begin{lemma}
    \label{lem:corner-pattern}
    Given a proper family $\RR$ with kernel rectangle $R_c$, there are at most $2$ corner rectangles, $N_i$ and $N_j$ containing a fixed corner of $R_c$. Furthermore, $N_i$ and $N_j$ pierce each other in a non-aligned way.
%  \end{lemma}
  \end{restatable}

  \begin{hproof}
    Refer to the $4$ cases shown in Figure~\ref{fig:corner-pattern}.
  \end{hproof}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  \hide{ %appendix
  \begin{proof}
  Let $N_i$ and $N_j$ be two corner rectangles, i.e., $N_i, N_j \in \RR_N$ and they contain the top-right corner of $R_c$. We do a case analysis below and conclude that $N_i$ and $N_j$ can only have a piercing intersection in a non-aligned way.
    \begin{enumerate}
    \item
      Assume $N_i$ and $N_j$ have a corner intersection between themselves. Without loss of generality, further assume that the left side of $N_i$ is to the left of that of $N_j$. There are two subcases. First, the top side of $N_i$ is above that of $N_j$. Second, the top side of $N_i$ is below that of $N_j$.

      In the first subcase, the left side of $N_j$ is completely in the interior of $N_i$ and $R_c$, which implies that $N_j$ is not area-maximal. Hence, contradiction (see Figure~\ref{fig:corner-pattern}, part $a$). In the second subcase, $N_j \cap R_c \cap \dP = \emptyset$ which implies $\RR$ is not a proper family, hence a contradiction again (see Figure~\ref{fig:corner-pattern}, part $b$).

    \item
      Assume $N_i$ and $N_j$ have a piercing intersection. The first subcase is that they are aligned to each other and the second subcase is that they are not.
      
      Without loss of generality, assume one of the side of $N_j$, $s_j$ is aligned to $s_i$, the corresponding side of $N_i$ and $s_j \subset s_i$. As $N_j$ is area-maximal, $s_j \cap \dP \neq \emptyset$. This also implies that $s_i \cap s_j \cap \dP \neq \emptyset$. Then it contradicts Observation~\ref{lem:corner-disjoint}
      (see Figure~\ref{fig:corner-pattern}, part $c$).

      For an example of $N_i$ and $N_j$ having a non-aligned piercing intersection, see part $d$ of Figure~\ref{fig:corner-pattern}.
      
    \end{enumerate}

    Next assume, that there is a third rectangle $N_k$ that also contains the top-right corner of $R_c$ and $N_i \prec N_k \prec N_j$. This implies $N_k \cap R_c \cap \dP = \emptyset$, which means $\RR$ is not proper and hence contradiction (see Figure~\ref{fig:corner-pattern}, part $d$).
      
  \end{proof}
}%\hide

  \begin{figure}[h]
        \centering
        \includegraphics[width=0.8\textwidth]{img/corner-pattern-flat}
        \caption{The subfigures are to support the various subcases of the proof of Lemma~\ref{lem:corner-pattern}. $\dP$ is drawn in thick red. The fill colors of rectangles $R_c, N_i, N_j, N_k$ are gray, red, blue, and green, respectively.}
        \label{fig:corner-pattern}
    \end{figure}


    As a consequence of Lemma~\ref{lem:corner-pattern}, we know that there are at most $8$ corner rectangles in $\RR$, at most $2$ per corner of $R_c$.
If there is a unique corner rectangle containing the top-right corner of $R_c$, we shall denote it by $N_{\nearrow}$. If there are two of them then we shall denote them by $N^v_\nearrow$ and $N^h_\nearrow$, where $N^v_\nearrow \prec N^h_\nearrow$. In general, a corner rectangle is denoted by $N^a_b$, where $a \in \{v,h,\emptyset\}$ and $b \in\{\swarrow, \nwarrow, \nearrow, \searrow\}$.
%    The corner rectangles, if any, containing the bottom-left corner, top-left corner, top-right corner, and right-bottom corner of $R_c$ are referred as $N_{\swarrow}, N_{\nwarrow}, N_{\nearrow},$ and $N_{\searrow}$, respectively.

  \subsection{Vertical and Horizontal Rectangles}
  We define the subset of maximally vertical rectangles with respect to the poset $\prec$ as $\RR^*_V := \max\{R \in \RR_V\}$. Similarly, we define the subset of minimally horizontal rectangles $\RR^*_H := \min\{R \in \RR_H\}$.

 
  \begin{restatable}[$\star$]{lemma}{VerticalTriple} 
  %\begin{lemma}
    \label{lem:vertical-triple}
There does not exist $3$ rectangles $R_i, R_j, R_k \in \RR^*_V$ (resp. $\RR^*_H$) such that each one has a corner intersection with the other two in $\dP$, i.e., $R_i \cap R_j \cap \dP \neq \emptyset$, $R_j \cap R_k \cap \dP \neq \emptyset$, and $R_i \cap R_k \cap \dP \neq \emptyset$.
%   \end{lemma}
    \end{restatable}


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \hide{ % appendix
  \begin{proof}
    Assume there exist $3$ rectangles, $R_i, R_j, R_k \in \RR$ such that $R_i \cap R_j \cap \dP \neq \emptyset$, $R_j \cap R_k \cap \dP \neq \emptyset$, and $R_i \cap R_k \cap \dP \neq \emptyset$.
    Combinatorially, triple of rectangles can be have pairwise corner intersection in two ways as shown in Figure~\ref{fig:vertical-triple}.
    If the triple intersect as shown on the left then $R_i \cap R_k \cap \dP = \emptyset$ which is a contradiction.
    If the triple intersect as shown on the right then the bottom side of $R_j$ and the right side of $R_i$ are completely in the interior of the union of the other two. This implies $R_i$ and $R_j$ are not area-maximal which is a contradiction.
  \end{proof}

}% hide appendix

 \begin{figure}[h]
        \centering
        \includegraphics[width=0.5\textwidth]{img/vertical-triple}
        \caption{Three rectangles can intersect in two ways such that every pair has a corner intersection.}
        \label{fig:vertical-triple}
    \end{figure}

    \begin{hproof}
      See Figure~\ref{fig:vertical-triple} to observe that there are combinatorially two ways in which a triple of area-maximal rectangles can have pairwise corner intersection. However, this leads to a contradiction.
    \end{hproof}
    
    
    Lemma~\ref{lem:vertical-triple} implies that we can linearly order the rectangles in $\RR^*_V$ (resp. $\RR^*_H$) as shown below.
    \begin{definition}
      \label{def:vert-order}
    Define a linear ordering $<_v$ on the rectangles in $\RR^*_V$, such that $R <_v R'$ if the left side of $R$ is to the left of that of $R'$, for every $R, R' \in \RR^*_V$.
  \end{definition}

  Let $\RR^*_V = \{V_1, \dots, V_k\}$, where $V_1 <_v \dots <_v V_k$.

  \begin{definition}
    \label{def:hori-order}
    Define a linear ordering $<_h$ on the rectangles in $\RR^*_H$, such that $R <_h R'$ if the bottom side of $R$ is below that of $R'$, for every $R, R' \in \RR^*_H$.
  \end{definition}

  Let $\RR^*_H = \{H_1, \dots, H_\ell\}$, where $H_1 <_h \dots <_h H_\ell$.

  \begin{restatable}[$\star$]{lemma}{Corpie}
   %\begin{lemma}
    \label{lem:2cor-1pie}
    Let $R_i, R_j \in \RR^*_V$ such that $R_i \cap R_j \cap \dP \neq \emptyset$. There does not exist $R_k \in \RR_V$ such that $R_k \prec R_i$ and $R_k \prec R_j$.
  %\end{lemma}
  \end{restatable}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \hide{ % appendix
  \begin{proof}
    Without loss of generality, assume $R_i <_v R_j$. For the sake of contradiction, lets assume such an $R_k$ exists. Then $R_k$ should be within the left side of $R_j$ and the right side of $R_i$ in order to have a piercing intersection with them. If $R_k$ is aligned to $R_i$ then they have an intersection with $\dP$ outside $R_c$, which means $R_c$ is not a kernel rectangle, hence a contradiction (see the left half of Figure~\ref{fig:vertical-consecutive}). Same is the case if it is aligned to $R_j$. If it is aligned to neither $R_i$ nor $R_j$, then $R_k \cap R_c \cap \dP = \emptyset$, which means $\RR$ is not proper, hence a contradiction again (see the right half of Figure~\ref{fig:vertical-consecutive}).
  \end{proof}

} % hide appendix

 \begin{figure}[h]
        \centering
        \includegraphics[width=0.65\textwidth]{img/vertical-consecutive}
        \caption{
          The above subfigures are to support Lemma~\ref{lem:2cor-1pie}.
        }
        \label{fig:vertical-consecutive}
    \end{figure}

    \begin{lemma}
      \label{lem:prec-star}
      Let $\RR^{\prec}_V(V_i) := \{R \in \RR_V \mid R \prec V_i\}$, for $V_i \in \RR^*_V$.
      There exists a support graph of $(\RR^{\prec}_V(V_i) \cup \{V_i\}, \dP)$ that is a star graph with $V_i$ as the center.
    \end{lemma}
    \begin{proof}
      Lemma~\ref{lem:2cor-1pie} implies that $V_i$ is a kernel rectangle of $(\RR^{\prec}_V(V_i) \cup \{V_i\}, \dP)$. Observation~\ref{lem:kernel-star} implies that the support graph of $(\RR^{\prec}_V(V_i) \cup \{V_i\}, \dP)$ is a star graph with $V_i$ as the center.
      \end{proof}
    Same arguments hold for $H_j \in \RR^*_H$.
    
  We refer $V_1, V_k, H_1,$ and $H_\ell$ to be terminal rectangles.

  If $V_1$ and $R_c$ have a common left blocker, then we call $V_1$ to be left-aligned. Likewise, if $V_k$ and $R_c$ have a common right blocker, then we call $V_k$ to be right-aligned. Conversely, if $H_1$ and $R_c$ have a common top blocker, then we call $H_1$ to be top-aligned. Finally, if $H_\ell$ and $R_c$ have a common bottom blocker, then we call $H_\ell$ to be bottom-aligned. Note that a terminal rectangle may or may not be aligned.


  \hide{
  \subsubsection*{Intersection across the Groups}
  % $\RR_N \times \RR_V$ (resp. $\RR_N \times \RR_H$)}
  \begin{lemma}
    If $R \cap R' \cap \dP \neq \emptyset$ such that the unordered pair $(R,R') \in (\RR_N\times\RR^*_V) \cup (\RR_N\times \RR^*_H) \cup (\RR^*_V \times \RR^*_H$) then $R$ and/or $R'$ are aligned.
  \end{lemma}
}

\subsection{Intersection between Corner and Non-corner Rectangles}

From Lemma~\ref{lem:corner} we know that any vertical or horizontal rectangle having an intersection with $N^a_\nearrow$ at $\dP$, should be top-aligned and/or right-aligned to $R_c$, where $a \in \{v,h,\emptyset\}$.

\begin{restatable}[$\star$]{lemma}{CornerNonCorner}
%\begin{lemma}
  \label{lem:corner-non-corner}
  There are at most $2$ vertical rectangles in $\RR^*_V$ and $2$ horizontal rectangles in $\RR^*_H$ intersecting a corner rectangle at $\dP$. Among these up to $4$ rectangles, there are at most $1$ vertical terminal rectangle, and at most $1$ horizontal terminal rectangle. Furthermore, for a fixed corner of $R_c$, if there are two corner rectangles, then there are at most $1$ vertical and $1$ horizontal rectangle per corner rectangle.
%\end{lemma}
\end{restatable}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hide{ % appendix
\begin{proof}
  Without loss of generality, fix the top-right corner of $R_c$. If there are corner rectangles, then either there is a single corner rectangle or there are two of them.

  For the first case, the corner rectangle is $N_\nearrow$ and there are possibly $4$ rectangles $V_i, V_k \in \RR^*_V$ and $H_j, H_\ell \in \RR^*_H$, where $1 \le i < k$ and $1 \le j < \ell$ such that they intersect $N_\nearrow$ at $\dP$. Recall that $V_k$ and $H_\ell$ are terminal rectangles (see Figure~\ref{fig:single-corner}).

  Similar is the case, if there are two corner rectangles, $N^v_\nearrow$ and $N^h_\nearrow$. $N^v_\nearrow$ has an intersection with $V_i$ and $H_\ell$ at a boundary point $p$, whereas, $N^h_\nearrow$ has an intersection with $V_k$ and $H_j$ at another boundary point $q$ (see Figure~\ref{fig:double-corner}).

\end{proof}

} % hide appendix

\begin{figure}[h]
  \centering
\begin{subfigure}[l]{0.49\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{img/single-corner-vert-hori}
        \caption{
          $N_\nearrow$ is the unique corner rectangle containing the top-right corner of $R_c$. Boundary points $p \in V_i \cap H_\ell \cap N_\nearrow \cap \dP$ and $q \in V_k \cap H_j \cap N_\nearrow \cap \dP$.
        }
        \label{fig:single-corner}
      \end{subfigure}
      \hfill
\begin{subfigure}[r]{0.49\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{img/pair-corner-vert-hori}
        \caption{
          $N^v_\nearrow$ and $N^h_\nearrow$ are the two corner rectangles containing the top-right corner of $R_c$.
          Boundary points $p \in V_i \cap H_\ell \cap N^h_\nearrow \cap \dP$ and $q \in V_k \cap H_j \cap N^v_\nearrow \cap \dP$.
        }
        \label{fig:double-corner}
      \end{subfigure}
      \caption{The intersection patterns between corner and non-corner rectangles.}
      \label{fig:single-double-corner}
    \end{figure}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    
    \hide{ % appendix
      
We make the following observation.

\begin{observation}
If there are two corner rectangles $N^v_b, N^h_b$ for a fixed corner $b$ of $R_c$, where $b = \{\nearrow, \nwarrow, \searrow, \swarrow\}$, then we can ignore $N^v_b$ and $N^h_b$ from our graph drawing algorithm.
\end{observation}

%If there are two corner rectangles $N^v_b, N^h_b$ for a fixed corner $b$ of $R_c$, where $b = \{\nearrow, \nwarrow, \searrow, \swarrow\}$, then
%As there are at most two rectangles $V_i$ and $H_j$, such that there exist $p \in \dP$ such that $p \in N^v_b \cap V_i \cap H_j \cap \dP \neq \emptyset$.
Note that the two edges $(N^v_b, V_i)$ and $(N^v_b, H_j)$ are enough to support  point $p$ in the support graph. Alternatively, we can ignore $N^v_b$, and instead consider drawing an edge joining vertices corresponding to $V_i$ and $H_j$ in the plane, and place a vertex corresponding to $N^v_b$ in the interior of the edge.
See Figure~\ref{fig:all-corners} for an illustration of all corners having two corner rectangles each, and also Figure~\ref{fig:graph-all-corners} for the corresponding support graph.
If only one of $V_i$ and $H_j$ exists then $N^v_b$ is a degree-$1$ vertex, and can be ignored as well.
Same arguments hold for $N^h_b$.

Also observe in Figure~\ref{fig:all-corners} if we replace $N^v_b$ and $N^h_b$ by $N_b$ such that the set of rectangles intersecting $N^v_b$ and $N^h_b$, intersects $N_b$ after replacement. Then in the Figure~\ref{fig:graph-all-corners}, the vertices corresponding to $N^v_b$ and $N^h_b$ can be contracted and the new vertex corresponds to $N_b$.

\begin{figure}[h]
        \centering
        \includegraphics[width=0.65\textwidth]{img/all-pair-corner-vert-hori}
        \caption{
          This figure is an extension of Figure~\ref{fig:double-corner} to all the $4$ corners of $R_c$. See Figure~\ref{fig:graph-all-corners} for the corresponding support graph.
        }
        \label{fig:all-corners}
\end{figure}

\begin{figure}[h]
  \centering \includegraphics[width=0.65\textwidth]{img/graph-all-corner-vert-hori}
        \caption{
          This figure shows the drawing of the support graph of the arrangement shown in Figure~\ref{fig:all-corners}.
          The edges drawn in solid lines are to support rectangles intersecting at $p_i$, $1 \le i \le 8$. Whereas the edges that do not involve corner rectangles are drawn in dashed lines.
        }
        \label{fig:graph-all-corners}
\end{figure}

} % hide appendix


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\hide{
\subsection{Algorithm to Draw Planar Support for $\RR\setminus ker(\RR)$}
We very briefly give an overview of our algorithm to draw a planar support of $(\RR\setminus ker(\RR), \dP)$. We place the vertices corresponding to the maximally horizontal rectangles, i.e., $\RR^*_H$ on a line in the same order as in $<_h$. Similarly we do the same for the rectangles in $\RR^*_V$.
Every vertex corresponding to a vertical (resp. horizontal) rectangle is made adjacent to a vertex corresponding to an aligned horizontal (resp. vertical) rectangle.
%  We put an edge between the left-aligned (resp.~right-aligned) rectangle, if it exists, and every horizontal rectangle. Similarly, we put an edge between the top-aligned (resp.~bottom-aligned) rectangle, if it exists, and every vertical rectangle. Without loss of generality, assume that all the aligned rectangles exist.
See Figure~\ref{fig:kernel-schema} for a schema of the drawing of $G$.
Refer to Subsection~\ref{sec:algo-kernel-less} in the appendices for the complete algorithm to draw planar support $G$ for $\RR\setminus ker(\RR)$.

  \hide{
  \subsubsection{Placing the vertices}
  Draw a circle and place the terminal vertices $V_1, H_1, V_k, H_\ell$ on it in this order i.e., alternating between the horizontal and vertical rectangles as shown in Figure~\ref{fig:kernel-schema} where the circle is drawn in bold.
  Place the vertices corresponding to the corner rectangle between the terminal rectangles, i.e.,
  $N_\swarrow$ between $V_1$ and $H_1$,
  $N_\searrow$ between $V_k$ and $H_1$,
  $N_\nearrow$ between $V_k$ and $H_\ell$, and
  $N_\nwarrow$ between $V_1$ and $H_\ell$.
  
  Define a line joining $H_1$ and $H_\ell$ in the inner face of the cycle. Place the vertices corresponding to the other horizontal rectangles $H_j \in \RR^*_H\setminus \{H_1, H_\ell\}$, on this line obeying the linear order defined in Definition~\ref{def:vert-order}.
  % and draw edges $(V_1,H_j)$ and $(V_k,H_j)$, for $1 < j < \ell$.
  Similarly, define a line joining $V_1$ and $V_k$ in the outer face of the cycle.
  Place the vertices corresponding to the other vertical rectangles $V_i \in \RR^*_V\setminus\{V_1, V_k\}$, on this line obeying the linear order defined in Definition~\ref{def:hori-order}.
  
  For every $V_i \in \RR^*_V$, if there exists $R$ such that $R \prec V_i$, then define a \emph{private} region in the plane (shown by a triangle with a vertex at $V_i$ in Figure~\ref{fig:kernel-schema}). Place the vertices corresponding to all such rectangles in the $V_i$'s private region.
  Similarly define private regions for $H_j \in \RR^*_H$, if required, and place all vertices corresponding to rectangles $R$ in the region, where $H_j \prec R$.

  \subsubsection{Drawing the edges}
  \begin{enumerate}
    \item {\bf $(\RR^*_V \times \RR^*_H)$.}
  If $V_1$ is left-aligned with $R_c$ then draw an edge $(V_1,H_j)$, for every $H_j \in \RR^*_H$ as shown in Figure~\ref{fig:kernel-schema}. Similarly, if $V_k$ is right-aligned then draw an edge $(V_k,H_j)$, for every $H_j \in \RR^*_H$.
  Conversely, if $H_1$ is bottom-aligned then draw an edge $(V_i, H_1)$, for every $V_i \in \RR^*_V$. Likewise, if $H_\ell$ is top-aligned then draw an edge $(V_i, H_\ell)$, for every $V_i \in \RR^*_V$.

\item {\bf $(\RR_V \times \RR_V)$.}
    If $V_i \cap V_{i+1} \cap \dP \neq \emptyset$ then draw an edge $(V_i,V_{i+1})$ for every $V_i \in \RR^*_V$ where $1 \le i < k$, along the line where the $V_i$'s are placed, as shown in Figure~\ref{fig:kernel-schema}.
  Draw an edge $(R,V_i)$ inside $V_i$'s private region, for every $V_i \in \RR^*_V$ and $R \prec V_i$.

\item {\bf $(\RR_H \times \RR_H)$.}
  If $H_j \cap H_{j+1} \cap \dP \neq \emptyset$ then draw an edge $(H_j,H_{j+1})$ for every $H_i \in \RR^*_H$ where $1 \le j < \ell$, along the line where the $H_j$'s are placed, as shown in Figure~\ref{fig:kernel-schema}.
  Draw an edge $(R,H_j)$ inside $H_j$'s private region, for every $H_j \in \RR^*_H$ and $H_j \prec R$.

\item {\bf $(\RR_N \times (\RR^*_V \cup \RR^*_H))$.}
  Lemma~\ref{lem:corner} implies that if $N_\nearrow \cap R \cap \dP \neq \emptyset$ where $R \in \RR^*_V \cup \RR^*_H$ then $R$ is either top-aligned and/or right-aligned to $R_c$. If $R$ is top-aligned to $R_c$ and $R \in \RR^*_H$ then $R = H_\ell$. Draw the edge $(N_\nearrow, H_\ell)$.
  If there exists $R' \in \RR^*_V$ such that $R' \cap N_\nearrow \cap \dP \neq \emptyset$ and $R'$ is top-aligned with $R_c$ then draw the edge $(N_\nearrow, R')$ if $N_\nearrow \cap H_\ell \cap \dP = \emptyset$, otherwise do not draw the edge $(N_\nearrow, R')$. See Figure~\ref{fig:kernel-corner}. The case where $R$ is top-aligned is identical and we accordingly draw the edges. Finally, we iterate over the other corner rectangles in $\RR_N$ and do a similar case analysis.
\end{enumerate}
}
  %$C_4$ and draw edges $(V_i, H_1)$ and $(V_i, H_k)$, for $1 < i < k$. If there exists corner rectangle intersecting a terminal rectangle, then we put an edge between them. See Figure~\ref{fig:kernel-schema}.



   \begin{SCfigure}[1][h]
        \centering
        \includegraphics[width=0.45\textwidth]{img/kernel-less-graph-schema}
        \caption{Schema of a planar support graph for $(\RR\setminus ker(\RR), \dP)$. $\RR^*_V = \{V_1,\dots, V_7\}$, $\RR^*_H = \{H_1, \dots, H_7\}$, $\RR_N = \{N_\swarrow, N_\nwarrow, N_\nearrow, N_\searrow\}$. For every $V_i \in \RR^*_V$, if there exists $R \prec V_i$, the vertex corresponding to $R$ is placed in the private triangular region attached to $V_i$. Likewise for vertices in $\RR^*_H$.}
        \label{fig:kernel-schema}
      \end{SCfigure}
      
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

      % \begin{restatable}{figure}{figabc}
      %   % \begin{figure}[h]
      %   \centering
      %   \includegraphics[width=0.65\textwidth]{img/kernel-corner}
      %   \caption{Schema of a planar support graph. $\RR^*_V = \{V_1,\dots, V_7\}$, $\RR^*_H = \{H_1, \dots, H_7\}$, $\RR_N = \{N_\swarrow, N_\nwarrow, N_\nearrow, N_\searrow\}$.
      %     In comparison to Figure~\ref{fig:kernel-schema}, here $H_7$ is not top-aligned and $V_5 \cap N_\nearrow \cap \dP \neq \emptyset$, hence there is the edge $(V_5, N_\nearrow)$.}
      %   \label{fig:kernel-corner}
      % %\end{figure}
      % \end{restatable}
      
%%%% Hiding the Algorithm
    \hide{
  \begin{algorithm}
    \caption{Algorithm to draw planar support for $(\RR\setminus ker(\RR), \dP)$}
    \label{alg:star}
    \begin{algorithmic}[1]
      \State Draw a circle $C$ on the plane.\;
      
      \State Draw the vertices corresponding to the terminal rectangles on $C$, in the order $V_1, H_1, V_k, H_\ell$. \;

      \State Draw the vertices corresponding to $V_2, \dots, V_{k-1}$ in the interior of $C$ along a line joining $V_1$ and $V_k$, respecting the linear ordering $<_v$. \;

      \State Draw the vertices corresponding to $H_2, \dots, H_{\ell -1}$ in the exterior of $C$ along some curved line joining $H_1$ and $H_\ell$, respecting the linear ordering $<_h$.\;

      \State Draw the vertex corresponding to $R_{11}$ on $C$ between $V_1$ and $H_1$.
      \If{$V_1 \cap R_{11} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{11},V_1)$.\;
      \EndIf
      \If{$H_1 \cap R_{11} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{11},H_1)$.\;
      \EndIf
      
      \State Draw the vertex corresponding to $R_{1 \ell}$ on $C$ between $V_1$ and $H_\ell$.
      \If{$V_1 \cap R_{1\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{1\ell},V_1)$.\;
      \EndIf
      \If{$H_\ell \cap R_{1\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{1\ell},H_\ell)$.\;
      \EndIf

      \State Draw the vertex corresponding to $R_{k1}$ on $C$ between $V_k$ and $H_1$.
      \If{$V_k \cap R_{k1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k1},V_k)$.\;
      \EndIf
      \If{$H_1 \cap R_{k1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k1},H_1)$.\;
      \EndIf
      
      \State Draw the vertex corresponding to $R_{k \ell}$ on $C$ between $V_k$ and $H_\ell$.
      \If{$V_k \cap R_{k\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k\ell},V_k)$.\;
      \EndIf
      \If{$H_\ell \cap R_{k\ell} \cap \dP \neq \emptyset$}
      \State Draw an edge $(R_{k\ell},H_\ell)$.\;
      \EndIf
      
      
      \If{$V_1$ is left-aligned}
      \ForAll{$H_j \in \RR^*_H$}
      \State Draw an edge $(V_1, H_j)$.
      \EndFor
      \EndIf

      \If{$V_k$ is right-aligned}
      \ForAll{$H_j \in \RR^*_H$}
      \State Draw an edge $(V_k, H_j)$.
      \EndFor
      \EndIf

      \If{$H_1$ is top-aligned}
      \ForAll{$V_i \in \RR^*_V$}
      \State Draw an edge $(V_i, H_1)$.
      \EndFor
      \EndIf

      \If{$H_\ell$ is bottom-aligned}
      \ForAll{$V_i \in \RR^*_V$}
      \State Draw an edge $(V_i, H_\ell)$.
      \EndFor
      \EndIf
      \algstore{myalg}
    \end{algorithmic}
  \end{algorithm}

  \begin{algorithm}                     
    \begin{algorithmic}% [1]
      \caption{Algorithm~\ref{alg:star} continued}
      \algrestore{myalg}
       
      \State $i \gets 1$\;
      \For{$i < k$}
      \If{$V_i \cap V_{i+1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(V_i, V_{i+1})$.\;
      \EndIf
      \State $i \gets i + 1$
      \EndFor

      \State $j \gets 1$\;
      \For{$j < \ell$}
      \If{$H_j \cap H_{j+1} \cap \dP \neq \emptyset$}
      \State Draw an edge $(H_j, H_{j+1})$.\;
      \EndIf
      \State $j \gets j + 1$
      \EndFor
      
    \end{algorithmic}
  \end{algorithm}

  } %End of hiding the algorithm.

  Finally, we state the remaining main lemma of this section.
  \begin{restatable}[$\star$]{lemma}{EtoileSansCentre}
  %\begin{lemma}
  \label{lem:etoile-sans-centre}
Given a family $(\RR, \dP)$ such that $ker(\RR) \neq \emptyset$, then $(\RR\setminus ker(\RR), \dP)$ has a planar support.
  %\end{lemma}
  \end{restatable}


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
  %%%%% MOVED TO APPENDIX %%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \hide{ %appendix
\begin{proof}

  It is easy to see with the help of Figures~\ref{fig:kernel-schema} and~\ref{fig:kernel-corner} that the resultant graph $G$ is planar.
  We claim that $G$ is also a support graph. For $p \in \dP$ consider $\RR_p \setminus \{R_c\}$.
  %If this set only contains vertical and horizontal rectangles then it is relatively easy to see that $p$ is supported.
  Consider $R, R' \in \RR_p \setminus \{R_c\}$. We claim $R$ and $R'$ are connected in $G$.
  \begin{enumerate}
    \item
  If $R, R' \in \RR_V$ then let $V, V' \in \RR^*_V$ such that $R \preceq V$ (i.e., $R \prec V$ or $R=V$) and $R' \preceq V'$. From Lemma~\ref{lem:prec-star}, $(R,V)$ and $(R',V')$ are edges in $G$. This also means $V$ and $V'$ must be consecutive in the ordering $<_v$ and hence they are adjacent in $G$. Thus, $R$ and $R'$ are connected in $G$. 
  Same is the case for $R, R' \in \RR_H$.
  
\item
  If $R \in \RR_V$ and $R' \in \RR_H$. Let $V \in \RR^*_V$ and $H \in \RR^*_H$ such that $R \prec V$ and $H \prec R'$. Then observe that either $V$ is a left/right aligned terminal rectangle or $H$ is a top/bottom aligned terminal rectangle, or both. In either cases, they $(H,V)$ is an edge in $G$. Hence, $R$ and $R'$ connected in $G$.

\item
  If $R \in \RR_N, R' \in \RR_V$. Without loss of generality, let $R = N_\nearrow$ and let $V \in \RR^*_V$ and $R \preceq V$. From Lemma~\ref{lem:corner} there are two cases, either $V$ is top-aligned with $R_c$ or right-aligned with $R_c$. In either cases, there is an edge drawn between $V$ and $N_\nearrow$. For the former case, see Figure~\ref{fig:kernel-corner}. For the latter case, see Figure~\ref{fig:kernel-schema}. Thus, $R$ and $N_\nearrow$ are connected. The other cases involving $\RR_N$ and $\RR_H$ are identical.
\end{enumerate}
 % It is also a support graph because if $R_i \cap R_j \cap \dP \neq \emptyset$ then we have an edge $(R_i, R_j)$ in our graph, for every $R_i, R_j \in \RR\setminus \{R_c\}$. From Observation~\ref{obs:int-supp}, an intersection graph is a support graph with respect to an intersecting family of sets.
\end{proof}

} % hide appendix


